Contexts Matter: An Empirical Study on Contextual Influence in Fairness Testing for Deep Learning Systems

Background: Fairness testing for deep learning systems has been becoming increasingly important. However, much work assumes perfect context and conditions from the other parts: well-tuned hyperparameters for accuracy; rectified bias in data, and mitigated bias in the labeling. Yet, these are often difficult to achieve in practice due to their resource-/labour-intensive nature. Aims: In this paper, we aim to understand how varying contexts affect fairness testing outcomes. Method:We conduct an extensive empirical study, which covers $10,800$ cases, to investigate how contexts can change the fairness testing result at the model level against the existing assumptions. We also study why the outcomes were observed from the lens of correlation/fitness landscape analysis. Results: Our results show that different context types and settings generally lead to a significant impact on the testing, which is mainly caused by the shifts of the fitness landscape under varying contexts. Conclusions: Our findings provide key insights for practitioners to evaluate the test generators and hint at future research directions.

==> Table/context.tex <==
\begin{table}[t!]
\caption{Context types and settings used in fairness testing. The \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green cells} indicate the chosen ones in our study.}

%The total number of articles with only one setting for all context types is 8(37).

\footnotesize
\centering
   % \setlength{\tabcolsep}{0.5mm}
    \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{l|l|l}
    \toprule
    \textbf{Type} & \textbf{Setting Count}& \textbf{\# Papers} \\
    \midrule
    \multirow{2}{*}{\text{Detect label bias}}
    &\text{single label bias}&\text{26}\\
    &\text{multiple label bias}&\text{5}\\
    \hline

    \multirow{2}{*}{\text{Detect selection bias}}
    &\text{single selection bias}&\text{17}\\
    &\text{multiple selection bias}&\text{11}\\
    \hline

    \multirow{2}{*}{\text{Test hyperparameter}}
    &\text{fixed hyperparameter}&\text{29}\\
    &\text{range hyperparameter}&\text{3}\\
    \hline
    \multirow{2}{*}{\text{Detect feature bias}}
    &\text{single feature bias}&\text{11}\\
    &\text{mixed fixed bias}&\text{10}\\
    \hline    
    \multirow{2}{*}{\text{Test repair algorithm}}
    &\text{multiple algorithm}&\text{17}\\
    &\text{fixed algorithm}&\text{1}\\
    \hline
    
    \multirow{2}{*}{\text{Test compression algorithms}}
    &\text{multiple algorithms}&\text{14}\\
    &\text{fixed algorithms}&\text{3}\\
    \bottomrule
    \end{tabular}

    \end{adjustbox}
    \label{tab:context}
\end{table}

==> Table/dataset-old.tex <==
\begin{table}
\caption{The real-world datatset used in fairness testing.}
\label{tb:dataset}
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{l|l|l|l}
\toprule
    \textbf{Dataset} & \textbf{Domain} & \textbf{Size} & \textbf{Sensitive Attribute(s)}\\
    \midrule
    \textsc{Adult ~\cite{adultdataset2017}} & Finance&$ 45,222$& Sex, Race, Age\\
   
    \textsc{Bank~\cite{bankdataset2014}} & Finance&$ 45,211$& Age, Marital\\
   
    \textsc{German~\cite{germancreditdataset1994}} & Finance&$ 1,000$& Sex, Age\\
   
    \textsc{Credit~\cite{defaultcreditdataset2016}} & Finance&$ 30,000$& Sex, Marital, Education\\
   
    \textsc{Compas~\cite{compasdataset2016}} & Criminology&$ 6,172$& Sex, Race\\
   
    \textsc{Law School~\cite{lawschooldataset1998}} & Education&$ 20,708$& Sex, Race\\
   
    \textsc{Student~\cite{studentperformancedataset2014}} & Education&$ 648$& Sex, Age\\
   
    \textsc{Crime~\cite{CommunitiesCrime2011}} & Criminology&$ 2,215$& Race, Age\\
   
    \textsc{Kdd-Census~\cite{misc_census-income_(kdd)_117}} & Criminology&$ 284,556$& Sex, Race\\
   
    \textsc{Dutch~\cite{dutchcensus2014}} & Finance&$ 60,420$& Sex\\
   
    \textsc{Diabetes~\cite{diabetes1994}} & Healthcare&$ 45,715$& Race\\
   
    \textsc{OULAD~\cite{oulad2017}} & Education&$ 21,562$& Race\\

    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> Table/definition.tex <==

\begin{table}
\caption{ the adopted fairness definitions on fairness testing.}
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{l|l|l}
\toprule
    \textbf{Fairness Definition}&\textbf{description} &\textbf{Papers}\\
    \midrule
    \text{Individual fairness}&\text{""} &\text{41}\\
\hline
    \text{Group fairness}&\text{"Protected groups and non-protected groups receive the same treatment"}&\text{12}\\
    \bottomrule
    
\end{tabular}
\end{adjustbox}
\label{tb:fairness}
\end{table}


==> Table/generator.tex <==
\begin{table}
\caption{The test generation techniques and their Hyperparameter setting. The \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green cells} indicate the chosen ones in our study.}
\centering
\setlength{\tabcolsep}{0.7mm}
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{l|l|l}
\toprule
    \textbf{Name} & \textbf{papers} & \textbf{Hyperparameter setting}\\
    \midrule  

    \rowcolor{teal!20}{\text{ADF~\cite{zhang2020white}}}&\text{15}&\text{randomly chosen parameter(cluster count,step size)}\\    
    \rowcolor{teal!20}{\text{Aeqitas~\cite{udeshi2018automated}}}&\text{13}&\text{randomly chosen parameter(cluster size,step size)}\\
    \rowcolor{teal!20}{\text{EIDIG~\cite{DBLP:conf/issta/ZhangZZ21}}}&\text{12}&\text{fixed settings(cluster size,step size,decay factor)}\\
    
    \text{SG~\cite{DBLP:conf/sigsoft/AggarwalLNDS19}}&\text{7}&\text{fixed settings(threshold,cluster size)}\\
    
    \text{THEMIS~\cite{DBLP:conf/sigsoft/GalhotraBM17}}&\text{5}&\text{fixed settings(threshold,cluster size}\\
    
    \text{ExpGA~\cite{DBLP:conf/icse/0002WJY022}}&\text{4}&\text{fixed settings(seed sample selection,crossover,mutation)}\\
    
    \text{NeuronFair~\cite{DBLP:conf/icse/ZhengCD0CJW0C22}}&\text{2}&\text{fixed setting(cluster size,seed size,decay rate,step size,perturbation size)}\\
    
    \text{DICE~\cite{DBLP:conf/icse/MonjeziTTT23}}&\text{1}&\text{fixed setting(h num epochs, batch size, and learning rate)}\\   
    
    \text{RULER~\cite{DBLP:conf/sigsoft/TaoSHF022}}&\text{1}&\text{fixed setting(cluster size,seed size,step size,perturbation size)}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\label{tb:generator}
\end{table}


==> Table/hp-setting-old.tex <==
\begin{table}[]
    \caption{Context settings for hyperparameters. $[R]$, $[N]$, and $[C]$ denote real, integer, and categorical values, respectively.}
       \centering
    \begin{adjustbox}{width=\linewidth,center}
    \begin{tabular}{l|l|l}
             \toprule
        % \multirow{2}{*}{\textbf{Name}}&\multicolumn{3}{c||}{\textbf{Hyperparameter}}
        \textbf{Parameter Name}&\textbf{Description} &  \textbf{Range}\\
     \midrule
           \text{learning\_rate$^{[R]}$}&Learning rate &$[10^{-6},10^{-1}]$\\
           \text{batch\_size$^{[N]}$}&Batch size&$\{2^4,2^5,...,2^{10}\}$\\
           \text{num\_epochs$^{[N]}$}&Number of epochs&$[50,200]$\\
           \text{num\_units$^{[N]}$}&Number of neurons&$\{2^4,2^5,...,2^{10}\}$\\
           \text{activation\_fn$^{[C]}$}&Activation function&$\{$ReLU, Sigmoid, Tah$\}$\\
           \text{optimizer$^{[C]}$}&Optimization algorithm &$\{$Adam, SGD$\}$\\
           \text{num\_layers$^{[N]}$}&Number of layers&$[2,10]$\\          \text{regularization\_param$^{[R]}$}&Regularization setting&$[10^{-5},10^{-1}]$\\
           \text{weight\_init\_method$^{[C]}$}&Weighting method&$\{$Random, Xavier, HE$\}$\\
           \bottomrule
    \end{tabular}
        \end{adjustbox}

    \label{tab:hp-setting}
\end{table}


==> Table/rq1-adq.tex <==

\begin{table*}[t!]
\caption{RQ1. Mean, standard error (SE), and scott knott rank $r$ for test adequacy metric. The best metric or lowest SE are denoted by \colorbox{green!20}{green cells}; \colorbox{red!20}{red cells} means the worst metric or highest SE.}
\label{tb:rq1}
\setlength{\tabcolsep}{0.7mm}
%\footnotesize
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc}\toprule

\multirow{2}{*}{\textbf{Dataset}}&\multicolumn{3}{c|}{\textbf{\texttt{Aequitas}  (\{$r$\} mean)}}&\multicolumn{3}{c|}{\textbf{\texttt{Aequitas} (SE)}}&\multicolumn{3}{c|}{\textbf{\texttt{ADF}  (\{$r$\}  mean)}}&\multicolumn{3}{c|}{\textbf{\texttt{ADF}  (SE)}}&\multicolumn{3}{c|}{\textbf{\texttt{EIDIG}  (\{$r$\}  mean)}}&\multicolumn{3}{c}{\textbf{\texttt{EIDIG}  (SE)}}\\


\cmidrule{2-19}

&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB\\

\midrule

Bank&\{\colorbox{green!20}{2.00}\} 0.47&\{\colorbox{red!20}{4.20}\} 0.31&\{3.80\} 0.37&$\pm$\colorbox{red!20} {0.41}&$\pm$ 0.36&$\pm$\colorbox{green!20} {0.34}&\{\colorbox{green!20}{1.60}\} 0.52&\{\colorbox{red!20}{4.00}\} 0.36&\{3.60\} 0.42&$\pm$\colorbox{red!20} {0.43}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.34} &\{\colorbox{green!20}{1.40}\} 0.67&\{\colorbox{red!20}{4.00}\} 0.45&\{3.60\} 0.53&$\pm$\colorbox{red!20}{0.38}&$\pm$\colorbox{green!20}{0.32}&$\pm $0.36\\

							
\midrule
Adult&\{\colorbox{green!20}{2.40}\} 0.57&\{3.80\} 0.36&\{\colorbox{red!20}{4.00}\} 0.44&$\pm$\colorbox{red!20}{0.43}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.34}&\{\colorbox{green!20}{1.80}\} 0.53&\{3.00\} 0.51&\{\colorbox{red!20}{3.40}\} 0.52&$\pm$\colorbox{red!20}{0.41}&$\pm$ 0.36&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.40}\} 0.55&\{3.20\} 0.53&\{\colorbox{red!20}{3.80}\} 0.51&$\pm$\colorbox{red!20}{0.46}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.35}\\
								


\midrule
Credit&\{\colorbox{green!20}{2.80}\} 0.46&\{\colorbox{red!20}{4.00}\} 0.30&\{3.60\} 0.38&$\pm$\colorbox{red!20}{0.37}&$\pm$\colorbox{green!20}{0.33}&$\pm$ 0.35&\{\colorbox{green!20}{2.40}\} 0.57&\{3.60\} 0.50&\{\colorbox{red!20}{4.60}\} 0.51&$\pm$\colorbox{red!20}{0.45}&$\pm$ \colorbox{green!20}{0.33}&$\pm$0.34&\{\colorbox{green!20}{1.40}\} 0.64&\{3.20\} 0.52&\{\colorbox{red!20}{3.80}\} 0.50&$\pm$\colorbox{red!20}{0.39}&$\pm$ \colorbox{green!20}{0.31}&$\pm$ 0.33\\
							
								
\midrule
German&\{\colorbox{green!20}{2.20}\} 0.39&\{\colorbox{red!20}{4.60}\} 0.30&\{3.60\} 0.31&$\pm$\colorbox{red!20}{0.45}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.37}&\{\colorbox{green!20}{1.80}\} 0.47&\{\colorbox{red!20}{4.40}\} 0.37&\{4.00\} 0.43&$\pm$\colorbox{red!20}{0.46}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.60}\} 0.56&\{\colorbox{red!20}{4.00}\} 0.51&\{3.60\} 0.52&$\pm$\colorbox{red!20}{0.44}&$\pm$ 0.35&$\pm$\colorbox{green!20}{0.32}\\

								

\midrule
Compas&\{\colorbox{green!20}{2.60}\} 0.48&\{3.60\} 0.42&\{\colorbox{red!20}{4.40}\} 0.44&$\pm$\colorbox{red!20}{0.45}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.36}&\{\colorbox{green!20}{1.20}\} 0.53&\{3.00\} 0.43&\{\colorbox{red!20}{3.40}\} 0.46&$\pm$\colorbox{red!20}{0.50}&$\pm$ 0.39&$\pm$\colorbox{green!20}{0.32}&\{\colorbox{green!20}{1.60}\} 0.58&\{\colorbox{red!20}{3.60}\} 0.49&\{3.40\} 0.53&$\pm$\colorbox{red!20}{0.48}&$\pm$ 0.42&$\pm$\colorbox{green!20}{0.36}\\



\midrule
Law School&\{\colorbox{green!20}{2.00}\} 0.53&\{\colorbox{red!20}{4.20}\} 0.39&\{3.60\} 0.46&$\pm$\colorbox{red!20}{0.52}&$\pm$ 0.44&$\pm$\colorbox{green!20}{0.37}&\{\colorbox{green!20}{2.00}\} 0.56&\{\colorbox{red!20}{3.60}\} 0.49&\{3.40\} 0.51&$\pm$\colorbox{red!20}{0.45}&$\pm$\colorbox{green!20}{0.33}&$\pm$ 0.41&\{\colorbox{green!20}{1.60}\} 0.61&\{\colorbox{red!20}{3.80}\} 0.53&\{3.40\} 0.56&$\pm$\colorbox{red!20}{0.43}&$\pm$\colorbox{green!20}{0.36}&$\pm$ 0.39\\
							
\midrule
Student&\{\colorbox{green!20}{2.80}\} 0.45&\{\colorbox{red!20}{4.20}\} 0.39&\{3.00\} 0.42&$\pm$\colorbox{red!20}{0.47}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.34}&\{\colorbox{green!20}{2.00}\} 0.54&\{\colorbox{red!20}{3.80}\} 0.46&\{3.20\} 0.49&$\pm$\colorbox{red!20}{0.46}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.60}\} 0.53&\{\colorbox{red!20}{3.60}\} 0.47&\{3.20\} 0.50&$\pm$\colorbox{red!20}{0.43}&$\pm$ 0.35&$\pm$\colorbox{green!20}{0.32}\\

						
\midrule
Crime&\{\colorbox{green!20}{1.60}\} 0.52&\{\colorbox{red!20}{4.40}\} 0.46&\{3.20\} 0.50&$\pm$\colorbox{red!20}{0.47}&$\pm$ 0.39&$\pm$\colorbox{green!20}{0.37}&\{\colorbox{green!20}{2.00}\} 0.56&\{\colorbox{red!20}{3.60}\} 0.52&\{2.40\} 0.54&$\pm$\colorbox{red!20}{0.49}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.80}\} 0.59&\{\colorbox{red!20}{3.80}\} 0.50&\{3.00\} 0.52&$\pm$\colorbox{red!20}{0.45}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.32}\\

				
\midrule
Kdd-Census&\{\colorbox{green!20}{2.20}\} 0.51&\{\colorbox{red!20}{4.20}\} 0.44&\{3.80\} 0.50&$\pm$\colorbox{red!20}{0.52}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.35}&\{\colorbox{green!20}{2.20}\} 0.53&\{\colorbox{red!20}{3.80}\} 0.43&\{\colorbox{red!20}{3.80}\} 0.51&$\pm$\colorbox{red!20}{0.46}&$\pm$\colorbox{green!20}{0.34}&$\pm$ 0.37&\{\colorbox{green!20}{1.40}\} 0.57&\{\colorbox{red!20}{3.60}\} 0.52&\{3.00\} 0.53&$\pm$\colorbox{red!20}{0.49}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.33}\\
					
\midrule
Dutch&\{\colorbox{green!20}{1.60}\} 0.49&\{3.80\} 0.43&\{\colorbox{red!20}{4.00}\} 0.47&$\pm$\colorbox{red!20}{0.53}&$\pm$\colorbox{green!20}{0.39}&$\pm$ 0.42&\{\colorbox{green!20}{1.80}\} 0.52&\{\colorbox{red!20}{3.60}\} 0.48&\{3.40\} 0.51&$\pm$\colorbox{red!20}{0.48}&$\pm$\colorbox{green!20}{0.36}&$\pm$ 0.41&\{\colorbox{green!20}{1.40}\} 0.56&\{3.40\} 0.51&\{\colorbox{red!20}{3.60}\} 0.52&$\pm$\colorbox{red!20}{0.46}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.34}\\

\midrule
Diabetes&\{\colorbox{green!20}{2.00}\} 0.43&\{\colorbox{red!20}{4.60}\} 0.36&\{4.00\} 0.39&$\pm$\colorbox{red!20}{0.44}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.34}&\{\colorbox{green!20}{1.60}\} 0.53&\{\colorbox{red!20}{3.80}\} 0.43&\{3.60\} 0.47&$\pm$\colorbox{red!20}{0.53}&$\pm$\colorbox{green!20}{0.39}&$\pm$ 0.42&\{\colorbox{green!20}{1.40}\} 0.58&\{\colorbox{red!20}{3.80}\} 0.53&\{3.60\} 0.55&$\pm$\colorbox{red!20}{0.47}&$\pm$ 0.39&$\pm$\colorbox{green!20}{0.34}\\

\midrule
OULAD&\{\colorbox{green!20}{2.40}\} 0.49&\{3.60\} 0.45&\{\colorbox{red!20}{4.60}\} 0.47&$\pm$\colorbox{red!20}{0.48}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.60}\} 0.54&\{\colorbox{red!20}{4.20}\} 0.49&\{3.60\} 0.52&$\pm$\colorbox{red!20}{0.51}&$\pm$ 0.41&$\pm$\colorbox{green!20}{0.37}&\{\colorbox{green!20}{1.80}\} 0.53&\{\colorbox{red!20}{4.00}\} 0.49&\{2.80\} 0.51&$\pm$\colorbox{red!20}{0.45}&$\pm$ 0.37&$\pm$\colorbox{green!20}{0.31}\\
					
% \midrule
% OVERALL&\{\colorbox{green!20}{2.22}\} 0.48&\{\colorbox{red!20}{4.10}\} 0.38&\{3.80\} 0.44&$\pm$\colorbox{red!20}{0.64}&$\pm$ 0.40&$\pm$\colorbox{green!20}{0.33}&\{\colorbox{green!20}{1.83}\} 0.54&\{\colorbox{red!20}{3.70}\} 0.46&\{3.53\} 0.49&$\pm$\colorbox{red!20}{0.66}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.32}&\{\colorbox{green!20}{1.53}\} 0.59&\{\colorbox{red!20}{3.67}\} 0.51&\{3.40\} 0.53&$\pm$\colorbox{red!20}{0.63}&$\pm$ 0.38&$\pm$\colorbox{green!20}{0.32}\\

%new-neg, Storm/RC = feature7
%\textsc{Trimesh}&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$\\




\bottomrule
\end{tabular}
\end{adjustbox}
%}
%\centering
 %\begin{tablenotes}
  %  \footnotesize
   % \item P and M denote the population size and the \# measurement search budget, respectively.
    %\end{tablenotes}
\end{table*}

==> Table/rq1-fair.tex <==

\begin{table*}[t!]
\caption{RQ1. Mean, standard error (SE), and scott knott rank $r$ for fairness metric. The best metric or lowest SE are denoted by \colorbox{green!20}{green cells}; \colorbox{red!20}{red cells} means the worst metric or highest SE. }
\label{tb:rq1}
\setlength{\tabcolsep}{0.7mm}
%\footnotesize
\centering
\begin{adjustbox}{width=\linewidth,center}
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc|ccc}\toprule

\multirow{2}{*}{\textbf{Dataset}}&\multicolumn{3}{c|}{\textbf{\texttt{Aequitas}  (\{$r$\} mean)}}&\multicolumn{3}{c|}{\textbf{\texttt{Aequitas} (SE)}}&\multicolumn{3}{c|}{\textbf{\texttt{ADF}  (\{$r$\}  mean)}}&\multicolumn{3}{c|}{\textbf{\texttt{ADF}  (SE)}}&\multicolumn{3}{c|}{\textbf{\texttt{EIDIG}  (\{$r$\}  mean)}}&\multicolumn{3}{c}{\textbf{\texttt{EIDIG}  (SE)}}\\

\cmidrule{2-19}

&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB&HP&SB&LB\\

\midrule

Bank&\{\colorbox{green!20}{1.80}\} 14.97&\{\colorbox{red!20}{3.80}\} 14.08&\{3.60\} 14.32&$\pm$\colorbox{red!20}{4.85}&$\pm$\colorbox{green!20}{2.54}&$\pm$ 4.63&\{\colorbox{green!20}{1.60}\} 15.41&\{3.40\} 14.92&\{\colorbox{red!20}{3.80}\} 15.13&$\pm$\colorbox{red!20}{3.86}&$\pm$\colorbox{green!20}{2.61}&$\pm$ 3.56&\{\colorbox{green!20}{1.40}\} 20.04&\{3.00\} 18.98&\{\colorbox{red!20}{3.20}\} 19.42&$\pm$\colorbox{red!20}{4.47}&$\pm$\colorbox{green!20}{2.44}&$\pm$ 3.66\\

		
       
\midrule
Adult&\{\colorbox{green!20}{2.20}\} 12.56&\{\colorbox{red!20}{4.00}\} 10.87&\{3.60\} 11.80&$\pm$\colorbox{red!20}{4.60}&$\pm$\colorbox{green!20}{2.84}&$\pm$ 3.47&\{\colorbox{green!20}{2.00}\} 13.46&\{\colorbox{red!20}{4.20}\} 13.02&\{3.40\} 13.13&$\pm$\colorbox{red!20}{3.90}&$\pm$\colorbox{green!20}{2.82}&$\pm$ 3.38&\{\colorbox{green!20}{1.40}\} 19.56&\{\colorbox{red!20}{3.80}\} 18.56&\{3.20\} 19.01&$\pm$\colorbox{red!20}{4.79}&$\pm$\colorbox{green!20}{2.89}&$\pm$ 3.59\\
								


\midrule
Credit&\{\colorbox{green!20}{2.60}\} 12.98&\{\colorbox{red!20}{4.20}\} 12.04&\{3.20\} 11.94&$\pm$\colorbox{red!20}{5.61}&$\pm$\colorbox{green!20}{3.11}&$\pm$ 3.74&\{\colorbox{green!20}{2.20}\} 14.54&\{\colorbox{red!20}{3.80}\} 13.93&\{3.60\} 14.21&$\pm$\colorbox{red!20}{4.25}&$\pm$\colorbox{green!20}{3.15}&$\pm$ 3.83&\{\colorbox{green!20}{1.20}\}22.50&\{\colorbox{red!20}{3.40}\} 21.04&\{3.20\} 21.51&$\pm$\colorbox{red!20}{4.29}&$\pm$\colorbox{green!20}{3.34}&$\pm$ 3.78\\
							
								
\midrule
German&\{\colorbox{green!20}{2.20}\} 11.52&\{\colorbox{red!20}{4.20}\} 10.55&\{3.60\} 11.03&$\pm$\colorbox{red!20}{3.63}&$\pm$\colorbox{green!20}{2.97}&$\pm$ 3.12&\{\colorbox{green!20}{2.00}\} 13.61&\{\colorbox{red!20}{3.80}\} 12.88&\{3.40\} 12.97&$\pm$\colorbox{red!20}{4.17}&$\pm$ 3.91&$\pm$\colorbox{green!20}{3.17}&\{\colorbox{green!20}{1.60}\} 21.40&\{3.40\} 20.58&\{\colorbox{red!20}{4.00}\} 20.89&$\pm$\colorbox{red!20}{3.67}&$\pm$\colorbox{green!20}{ 3.04}&$\pm$ 3.45\\

								

\midrule
Compas&\{\colorbox{green!20}{2.60}\} 12.43&\{\colorbox{red!20}{4.40}\} 11.39&\{3.80\} 11.55&$\pm$\colorbox{red!20}{4.78}&$\pm$\colorbox{green!20}{3.07}&$\pm$ 3.73&\{\colorbox{green!20}{1.80}\} 12.98&\{3.60\} 12.51&\{\colorbox{red!20}{4.00}\} 12.55&$\pm$\colorbox{red!20}{3.92}&$\pm$\colorbox{green!20}{3.03}&$\pm$ 3.66&\{\colorbox{green!20}{1.6}0\} 20.45&\{\colorbox{red!20}{3.80}\} 19.37&\{3.40\} 19.88&$\pm$\colorbox{red!20}{4.76}&$\pm$\colorbox{green!20}{3.07}&$\pm$ 4.07\\



\midrule
Law School&\{\colorbox{green!20}{2.20}\} 12.99&\{\colorbox{red!20}{4.20}\} 11.29&\{3.80\} 11.49&$\pm$\colorbox{red!20}{4.22}&$\pm$\colorbox{green!20}{3.16}&$\pm$ 3.90&\{\colorbox{green!20}{2.80}\} 12.43&\{\colorbox{red!20}{4.00}\} 11.97&\{3.60\} 12.03&$\pm$ 3.96&$\pm$\colorbox{green!20}{3.20}&$\pm$\colorbox{red!20}{4.92}&\{\colorbox{green!20}{1.80}\} 21.49&\{3.60\} 19.53&\{\colorbox{red!20}{3.8 }\} 20.54&$\pm$\colorbox{red!20}{3.84}&$\pm$\colorbox{green!20}{3.14}&$\pm$ 3.67\\
							
\midrule
Student&\{\colorbox{green!20}{2.60}\} 13.93&\{3.80\} 12.43&\{\colorbox{red!20}{4.00}\} 12.56&$\pm$\colorbox{red!20}{4.54}&$\pm$ 2.55&$\pm$\colorbox{green!20}{3.71}&\{\colorbox{green!20}{2.20}\} 14.88&\{3.60\} 14.50&\{\colorbox{red!20}{3.80}\} 14.57&$\pm$\colorbox{red!20}{4.83}&$\pm$\colorbox{green!20}{2.52}&$\pm$ 3.77&\{\colorbox{green!20}{1.20}\} 22.08&\{\colorbox{red!20}{3.40}\} 20.91&\{3.20\} 21.60&$\pm$\colorbox{red!20}{3.94}&$\pm$\colorbox{green!20}{3.12}&$\pm$ 3.83\\

						
\midrule
Crime&\{\colorbox{green!20}{1.60}\} 12.95&\{\colorbox{red!20}{4.00}\} 11.97&\{3.40\} 12.42&$\pm$\colorbox{red!20}{4.04}&$\pm$\colorbox{green!20}{3.36}&$\pm$3.62&\{\colorbox{green!20}{1.80}\} 15.39&\{3.40\} 15.01&\{\colorbox{red!20}{3.80}\} 15.08&$\pm$\colorbox{red!20}{3.69}&$\pm$\colorbox{green!20}{3.39}&$\pm$ 3.42&\{\colorbox{green!20}{1.40}\} 21.85&\{\colorbox{red!20}{3.40}\} 20.94&\{3.00\} 21.55&$\pm$\colorbox{red!20}{4.76}&$\pm$\colorbox{green!20}{2.54}&$\pm$ 3.76\\


\midrule
Kdd-Census&\{\colorbox{green!20}{2.40}\} 13.42&\{\colorbox{red!20}{4.20}\} 12.42&\{3.60\} 12.39&$\pm$\colorbox{red!20}{4.28}&$\pm$\colorbox{green!20}{3.14}&$\pm$ 3.37&\{\colorbox{green!20}{2.00}\} 16.47&\{\colorbox{red!20}{3.80}\} 15.52&\{3.40\} 15.88&$\pm$\colorbox{red!20}{4.22}&$\pm$\colorbox{green!20}{3.25}&$\pm$ 3.68&\{\colorbox{green!20}{1.60}\} 23.57&\{\colorbox{red!20}{3.40}\} 22.51&\{3.00\} 22.94&$\pm$\colorbox{red!20}{3.72}&$\pm$ 3.43&$\pm$\colorbox{green!20}{3.36}\\



\midrule
Dutch&\{\colorbox{green!20}{2.60}\} 13.47&\{3.20\} 13.01&\{\colorbox{red!20}{3.80}\} 12.98&$\pm$\colorbox{red!20}{3.76}&$\pm$\colorbox{green!20}{3.16}&$\pm$ 3.44&\{\colorbox{green!20}{2.40}\} 14.53&\{\colorbox{red!20}{4.20}\} 14.04&\{3.20\} 14.36&$\pm$\colorbox{red!20}{3.66}&$\pm$\colorbox{green!20}{3.27}&$\pm$ 3.40&\{\colorbox{green!20}{1.40}\} 21.75&\{3.20\} 20.88&\{\colorbox{red!20}{3.40}\} 21.60&$\pm$\colorbox{red!20}{4.32}&$\pm$\colorbox{green!20}{3.03}&$\pm$ 3.63\\


\midrule
Diabetes&\{\colorbox{green!20}{2.20}\} 13.51&\{4.20\} 12.52&\{\colorbox{red!20}{4.60}\} 12.63&$\pm$\colorbox{red!20}{4.29}&$\pm$ 2.56&$\pm$\colorbox{green!20}{3.79}&\{\colorbox{green!20}{1.80}\} 13.56&\{\colorbox{red!20}{3.80}\} 12.97&\{3.60\} 13.36&$\pm$\colorbox{red!20}{4.54}&$\pm$\colorbox{green!20}{2.52}&$\pm$ 3.62&\{\colorbox{green!20}{1.40}\} 19.52&\{\colorbox{red!20}{3.20}\} 19.05&\{2.80\} 19.56&$\pm$\colorbox{red!20}{4.18}&$\pm$ 3.43&$\pm$\colorbox{green!20}{3.41}\\
					

\midrule
OULAD&\{\colorbox{green!20}{2.40}\} 12.97&\{3.80\} 12.04&\{\colorbox{red!20}{4.20}\} 12.52&$\pm$\colorbox{red!20}{4.60}&$\pm$\colorbox{green!20}{3.33}&$\pm$ 3.45&\{\colorbox{green!20}{1.80}\} 13.01&\{3.40\} 12.47&\{\colorbox{red!20}{4.20}\} 12.92&$\pm$\colorbox{red!20}{3.93}&$\pm$\colorbox{green!20}{3.23}&$\pm$ 3.53&\{\colorbox{green!20}{1.60}\} 23.04&\{\colorbox{red!20}{4.00}\} 22.09&\{3.20\} 22.44&$\pm$\colorbox{red!20}{3.88}&$\pm$\colorbox{green!20}{3.36}&$\pm$ 3.47\\

% \midrule
% OVERALL&\{\colorbox{green!20}{2.28}\} 0.49&\{\colorbox{red!20}{4.00}\} 0.45&\{3.77\} 0.47&$\pm$\colorbox{red!20}{5.85}&$\pm$\colorbox{green!20}{3.31}&$\pm$ 3.61&\{\colorbox{green!20}{2.03}\}0.52&\{\colorbox{red!20}{3.75}\} 0.48&\{3.65\} 0.50&$\pm$\colorbox{red!20}{5.93}&$\pm$\colorbox{green!20}{3.36}&$\pm$ 3.86&\{\colorbox{green!20}{1.46}\} 0.55&\{\colorbox{red!20}{3.47}\} 0.50&\{3.28\} 0.53&$\pm$\colorbox{red!20}{6.08}&$\pm$\colorbox{green!20}{3.35}&$\pm$ 4.01\\


	
	
	


%new-neg, Storm/RC = feature7
%\textsc{Trimesh}&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$&0.21$_{\pm0.02}$&0.33$_{\pm0.02}$\\ 




\bottomrule
\end{tabular}
\end{adjustbox}
%}
%\centering
 %\begin{tablenotes}
  %  \footnotesize
   % \item P and M denote the population size and the \# measurement search budget, respectively.
    %\end{tablenotes}
\end{table*}

==> background-old.tex <==
\section{background}
\label{sec:pre}

\textcolor{red}{Group fairness is defining that machine learning models should give equal treatment to different populations or predefined groups. Also known as demographic fairness or statistical fairness, it looks at achieving fairness in the model output at an overall level. This requires that the model should not favour any one group because of protected characteristics such as age, gender, race or religion. For example, in a candidate screening scenario, group fairness means that different demographic groups should have roughly equal acceptance rates. While this approach ensures fairness at the broad demographic level, it may ignore differences between individuals within groups.}

\textcolor{red}{Individual fairness is the notion that similar individuals should be treated in a similar manner by machine learning models. The micro-conceptual definition of this concept, where the definition of "similar" depends on the specific scenario. For example, in a loan approval system, two applicants with similar credit histories, income levels, and financial habits should be awarded the same loan amount or interest rate. Individual fairness aims to create fair consistency tailored to each situation, thus ensuring that the model makes fair decisions at the individual level.}
\subsection{Test Components}
Fairness testing is a critical process in evaluating and ensuring the fairness of machine learning models, particularly in the context of decision-making systems. As AI systems become more prevalent in various domains, it is crucial to assess whether these systems exhibit discriminatory behavior or bias towards certain groups or individuals based on protected attributes such as race, gender, or age\cite{tao2022ruler,bastani2019probabilistic}. Ensuring fairness in AI systems is essential for promoting equal opportunities, avoiding unjust discrimination, and upholding ethical standards.

The first test component, label bias\cite{peng2021xfair,chen2021understanding,compasdataset2016}, refers to the presence of biased or unfair labels in the training data. Biases in labels can arise due to historical or societal biases, flawed data collection processes, or the subjective nature of label assignment. Label bias can significantly impact the fairness of a DNN model, as it may perpetuate or amplify existing biases in the training data. Assessing and mitigating label bias is crucial to ensure fair and unbiased decision-making by the model.

The second test component, select bias\cite{yeom2021avoiding,chakraborty2022fairssl,karkkainen2021fairface}, pertains to biases that arise during the process of selecting features or variables used for model training. Feature selection is a critical step in building machine learning models, as it determines which attributes of the data are considered for making predictions. However, if the selection process is biased or discriminates against certain groups, the resulting model may inherit and perpetuate those biases. Analyzing select bias helps identify and address discriminatory feature selection practices, enabling the development of fairer models.

The third test component, hyperparameter tuning\cite{chakraborty2019software,corbett2017algorithmic,nair2020finding,zhang2022fairness}, focuses on the optimization of model performance by adjusting hyperparameters, such as learning rates, regularization parameters, or network architectures. While hyperparameter tuning is aimed at improving model accuracy and generalization, it can inadvertently introduce biases or unfairness. Certain combinations of hyperparameters may result in models that favor specific groups or exhibit discriminatory behavior. Understanding the impact of hyperparameter tuning on fairness is crucial to ensure that model optimization does not compromise fairness principles.

\subsection{Test Input Generation}
Individual fairness testing is a crucial aspect of evaluating and addressing potential discrimination in machine learning models. This process involves mutating input samples to generate a sufficient number of testing samples and assessing whether these samples exhibit individual-discriminatory behavior\cite{zhang2023rethinking}. Several typical approaches have been developed for individual fairness testing, including THEMIS\cite{udeshi2018automated}, AEQUITAS\cite{galhotra2017fairness}, SG\cite{aggarwal2019black}, ADF\cite{zhang2021fairness}, and EIDIG\cite{zheng2022neuronfair}.

In general, these fairness testing methods follow a similar workflow. They begin by constructing a set of seed samples that are suspiciously discriminatory. These seed samples are generated using random or clustering techniques\cite{hardy2021fairness}. The goal is to identify initial instances that may showcase discriminatory patterns in the model's behavior. Once the seed samples are obtained, the methods employ different strategies to search for additional discriminatory samples around these seeds.

One common strategy used in fairness testing is symbolic execu-tion\cite{chen2021fairness,aggarwal2019black}. Symbolic execution involves exploring the different execution paths and conditions within a model to uncover discriminatory behaviors. By traversing the model's decision-making process symbolically, these methods can identify inputs or features that lead to biased outcomes. This allows for the detection of discriminatory samples that may have been overlooked during the initial seed generation phase.

Another strategy employed in fairness testing is gradient-based methods\cite{zheng2022neuronfair,zhang2021fairness,zhang2020white}. These methods leverage the gradient information of the model to identify discriminatory patterns. By analyzing the gradients of the model with respect to the input features, it becomes possible to identify instances where small perturbations in the input can significantly alter the model's predictions and potentially lead to biased outcomes\cite{he2022deep}. This approach allows for a more fine-grained exploration of the model's behavior and can uncover subtle discriminatory tendencies.

Figure 1 briefly illustrates our experimental design.
First, we use 12 widely adopted datasets to train the DeepLearning model. Second, we introduce three different background cases during model training (adjusting label bias and select bias in the dataset during the data preprocessing phase and adjusting the training model hyperparameters during the training model setup). Third, we use 5 adequacy metrics and 1 individual fairness metric to evaluate the different methods.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/Workflow.pdf}
    \caption{The Workflow of this study}
    \label{fig:my_fig}
\end{figure}

%Unlike traditional analytical models, machine learning based modeling takes a black-box manner that relies on observing a small amount of the software’s actual behaviors under certain conditions, in order to infer a statistical model to predict the performance without heavy human intervention~\cite{DBLP:books/daglib/0020252}. This is also what enable it to overcome the issues of heavy assumptions on the configuration options and the system's characteristics in analytical models~\cite{DBLP:journals/tse/YuWHH19,DBLP:conf/splc/TempleAPBJR19,DBLP:journals/tosem/ChenLBY18,DBLP:journals/corr/abs-1801-02175}.

\subsection{Some Metrics}
In the context of fairness testing, adequacy metrics play a crucial role in guiding the testing process and evaluating the fairness of machine learning models. These metrics provide quantitative measures of how well the testing inputs explore the space of potential biases and discriminatory behavior. 
In this section, we will introduct five adequacy metrics commonly used in fairness testing\cite{zhang2022deep,khatibsyarbini2019test,amazon2016unbiased}: Distance-based Surprise Adequacy (DSA)\cite{karkkainen2021fairface},Likelihood-based Surprise Adequacy (LSA)\cite{ma2018deepgauge}, Neuron Coverage (NC)\cite{hitaj2017deep}, Neuron Boundary Coverage (NBC)\cite{chen2020comprehensive}, and Strong Neuron Activation Coverage(SNAC)\cite{galhotra2017fairness}.
\subsubsection{Likelihood-based Surprise Adequacy(LSA)}
\begin{itemize}
  \item Likelihood-based Surprise Adequacy (LSA)\cite{ma2018deepgauge}. Let $\alpha_{o}(x)$ denote the activation value of a single neuron $o$ with respect to an input $x$. For a set of neurons in a layer of the DNN, denoted as $O^{\prime} \subseteq O$, $\alpha_{O^{\prime}}(x)$ denotes a vector of activation values that represents the Activation Trace (AT) of $x$ over neurons in $O^{\prime}$. For a set of inputs $X, A_{O^{\prime}}(X)=\left\{\alpha_{O^{\prime}}(x) \mid x \in X\right\}$ denotes the set of activation traces observed for neurons in $O^{\prime}$. Given a training set $T$, a bandwidth matrix $H$ and a Gaussian kernal function $K$, the activation trace of a new input $x, \mathrm{KDE}$ produces a density function $\hat{f}$ as follows.
\end{itemize}

$$
\hat{f}(x)=\frac{1}{\left|A_{O^{\prime}}(T)\right|} \sum_{x_{i} \in T} K_{H}\left(\alpha_{O^{\prime}}(x)-\alpha_{O^{\prime}}\left(x_{i}\right)\right)
$$

Intuitively, the function measures a normalized distance between the activation values of $x$ and those of individual inputs in $T$ (regarding $O^{\prime}$ ). Then LSA is defined as follows.

$$
\operatorname{LSA}(x)=-\log (\hat{f}(x))
$$
\subsubsection{Distance-based Surprise Adequacy(DSA)}
\begin{itemize}
  \item Distance-based Surprise Adequacy (DSA)\cite{karkkainen2021fairface}. Assume a DL system $F$, which consists of a set of neurons $O$, is trained for a classification task with a set of classes $Y$, using a training dataset $T$. Given the set of activation traces $A_{O}(T)$, a new input $x$, and a predicted class of the new input $C \in Y$. The closest neighbor of $x$ that shares the same output class, denoted as $x_{a}$, and their distance, are defined as follows.
\end{itemize}

$$
\begin{aligned}
& x_{a}=\underset{F\left(x_{i}\right)=y}{\operatorname{argmin}}\left\|\alpha_{O}(x)-\alpha_{O}\left(x_{i}\right)\right\| \\
& \operatorname{dist}_{a}=\left\|\alpha_{O}(x)-\alpha_{O}\left(x_{a}\right)\right\|
\end{aligned}
$$

The closest neighbor in a class other than $y$, denoted by $x_{b}$, and their distance $\operatorname{dist}_{b}$, are defined as follows.

$$
\begin{aligned}
& x_{b}=\underset{F\left(x_{i}\right) \in Y \backslash\{y\}}{\operatorname{argmin}}\left\|\alpha_{O}(x)-\alpha_{O}\left(x_{i}\right)\right\| \\
& \text { dist }_{b}=\left\|\alpha_{O}(x)-\alpha_{O}\left(x_{b}\right)\right\|
\end{aligned}
$$

Then the DSA is defined in the following. Intuitively, it measures if $x$ is closer to the target class or a different class.
$$\operatorname{DSA}(x)= \frac{\text { dist }_{a}}{\text { dist }_{b}}$$
\subsubsection{Neuron Coverage(NC)}
\begin{itemize}
  \item NC \cite{hitaj2017deep}is a coverage-based adequacy metric that focuses on the activation patterns of neurons in a deep learning model. It measures the percentage of neurons that are activated by the testing samples. The rationale behind NC is that discriminatory behaviors often manifest in the activation patterns of specific neurons. By ensuring high neuron coverage, fairness testing aims to explore the model's behavior comprehensively and capture discriminatory tendencies. Higher NC values indicate a more thorough exploration of the model's neuron activations and potential biases.
\end{itemize}
$$ N C=\frac{|A N|}{|O|} $$
$O$ is the universal set of neurons of a DNN.$AN$ is activated neuron.
\subsubsection{Neuron Boundary Coverage (NBC)}
\begin{itemize}
    \item NBC \cite{chen2020comprehensive}is a variation of the neuron coverage metric that specifically targets the boundaries between different classes or labels. It measures the coverage of neurons that are close to the decision boundaries of the model. NBC recognizes that discriminatory behaviors often occur near decision boundaries, where small changes in input can lead to different predictions. By focusing on these critical areas, NBC aims to uncover biases that may have significant impacts on decision-making. Higher NBC values indicate a more comprehensive exploration of decision boundaries and potential discriminatory behaviors.
\end{itemize}
$$
N B C=\frac{|U C N|+|L C N|}{2 \times|O|}
$$
$L C N$ is a set of activated neurons that fall in the corner-case regions, $U C N$ is a set of activated neurons that fall in the corner-case regions.
\subsubsection{Strong Neuron Activation Coverage(SNAC)}
\begin{itemize}
    \item SNAC\cite{campolo2017bias} is another extension of the neuron coverage concept. It not only considers whether a neuron is activated but also how strongly it is activated. High SNAC indicates that the model's neurons are not just being used, but they're also being used to their full potential.
\end{itemize}
$$
S N A C=\frac{|U C N|}{|O|}
$$

\subsubsection{Individual Discriminatory Instance(IDI)}
The concept of fairness in machine learning involves ensuring that models do not discriminate or create disparate outcomes based on protected attributes like race, gender, age, or disability\cite{zhang2022fairness,zheng2022neuronfair}. While many fairness metrics focus on group-based fairness, it's also critical to consider individual fairness to ensure that similar individuals are treated similarly.
\begin{itemize}
    \item The Individual Discriminatory Instance (IDI) metric is an example of a fairness measure that operates at the individual level.
    IDI is a measure of the extent to which an individual instance is treated unfairly by a machine learning model. It specifically captures instances where a model's output would change if some protected attribute of the instance were altered, while all other non-protected attributes remained the same.
\end{itemize}
    Let $X$ be a dataset with a set of attributes $A=\left\{a_{i} \mid i \in\{1, \ldots, n\}\right\}$. If $a_{i} \in \mathbb{I}_{i}$ holds for $1 \leq i \leq n$, the input domain of the corresponding decisionmaking software $\mathcal{S}: \mathbb{I} \rightarrow\{$ True, False $\}$ is $\mathbb{I}=\mathbb{I}_{1} \times \mathbb{I}_{2} \times \ldots \times \mathbb{I}_{n}$. We use $P$ to denote the set of protected attributes, and thus $A \backslash P$ is the set of non-protected attributes. We define that an instance $x \in \mathbb{I}$ is an individual discriminatory instance for software $\mathcal{S}$ if there exists an instance $x^{\prime} \in \mathbb{I}$ such that

\begin{itemize}
  \item $\exists a \in P, x_{a} \neq x_{a}^{\prime}$

  \item $\forall a \in A \backslash P, x_{a}=x_{a}^{\prime}$

  \item - $\mathcal{S}(x) \neq \mathcal{S}\left(x^{\prime}\right)$
\end{itemize}


The tuple $\left(x, x^{\prime}\right)$ is thus an individual discriminatory instance pair.
$$
IDI =\frac{GeneratedIDIsamples}{instancesrandomlysampled}
$$
% \begin{itemize}
%     \item Distance-based Surprise Adequacy (DSA):DSA is an adequacy metric that focuses on identifying discriminatory behavior towards protected attributes such as race or gender. It combines search-based testing techniques with discrimi-nation-awareness to guide the generation of test inputs. The goal is to ensure that the generated inputs cover different subgroups defined by the protected attributes and capture potential instances of discrimination. DSA takes into account the representation and distribution of subgroups in the dataset and aims to generate test inputs that explore various combinations of attributes to uncover biased predictions.
    
%     \item Likelihood-based Surprise Adequacy (LSA):LSA is an adequacy metric that measures the surprise factor of a testing sample. It assesses how unexpected a particular sample is to the model's predictions. LSA is based on the principle that discriminatory behavior often results in unexpected outcomes. By comparing the likelihood of a sample's predicted label to the likelihood of the true label, LSA quantifies the surprise caused by the model's prediction. Higher LSA values indicate that the model's behavior is less predictable and potentially more discriminatory.
    
%     \item Neuron Coverage (NC):
%     NC is a coverage-based adequacy metric that focuses on the activation patterns of neurons in a deep learning model. It measures the percentage of neurons that are activated by the testing samples. The rationale behind NC is that discriminatory behaviors often manifest in the activation patterns of specific neurons. By ensuring high neuron coverage, fairness testing aims to explore the model's behavior comprehensively and capture discriminatory tendencies. Higher NC values indicate a more thorough exploration of the model's neuron activations and potential biases.
    
%     \item Neuron Boundary Coverage (NBC):NBC is a variation of the neuron coverage metric that specifically targets the boundaries between different classes or labels. It measures the coverage of neurons that are close to the decision boundaries of the model. NBC recognizes that discriminatory behaviors often occur near decision boundaries, where small changes in input can lead to different predictions. By focusing on these critical areas, NBC aims to uncover biases that may have significant impacts on decision-making. Higher NBC values indicate a more comprehensive exploration of decision boundaries and potential discriminatory behaviors.
    
%     \item Strong Neuron Activation Coverage (SNAC):SNAC is another extension of the neuron coverage concept. It not only considers whether a neuron is activated but also how strongly it is activated. High SNAC indicates that the model's neurons are not just being used, but they're also being used to their full potential.
    
%     \item Individual Discriminatory Instance (IDI):The concept of fairness in machine learning involves ensuring that models do not discriminate or create disparate outcomes based on protected attributes like race, gender, age, or disability. While many fairness metrics focus on group-based fairness, it's also critical to consider individual fairness to ensure that similar individuals are treated similarly.
%     The Individual Discriminatory Instance (IDI) metric is an example of a fairness measure that operates at the individual level.
%     IDI is a measure of the extent to which an individual instance is treated unfairly by a machine learning model. It specifically captures instances where a model's output would change if some protected attribute of the instance were altered, while all other non-protected attributes remained the same.
%     For example, let's consider a machine learning model used in hiring. Suppose this model, given two applicants who are identical in every aspect except gender, consistently rates one gender higher than the other. In such a case, the model would have a high IDI score, indicating discriminatory behavior at the individual level.
% \end{itemize}

\subsection{FITNESS LANDSCAPE ANALYSIS Metric}

\subsubsection{Fitness Distance Correlation.}
Fitness Distance Correlation (FDC) measures the correlation of a solution's fitness and its distance to a global optimum \cite{tavares2008multidimensional,chen2022planning}. In minimization problems, a positive correlation indicates that the closer a solution distance is to the global optimum, the higher quality (i.e., lower cost) the solution has. The algorithm can benefit from such a fitness landscape and be more easily guided to the global optimum. In contrast, an instance with a negative correlation will potentially guide the algorithm towards the opposite direction of the global optimum. For DCARP instances, suppose $F=\left\{c_{1}, c_{2}, \ldots, c_{n}\right\}$ and $D=\left\{d_{1}, d_{2}, \ldots, d_{n}\right\}$ are the fitnesses of $n$ solutions and the distances to the global optimum of these solutions. FDC is calculated by the following equation [4]:

$$
F D C=\frac{\frac{1}{n} \sum_{i=1}^{n}\left(c_{i}-\bar{c}\right)\left(d_{i}-\bar{d}\right)}{\sigma_{F} \sigma_{D}}
$$

where $\sigma_{F}, \sigma_{D}, \bar{c}, \bar{d}$ represent the standard deviations and means of $F$ and $D$. The distance between two solutions are also measured by the Hamming distance as introduced in Section 4.3.4. The mean FDCs over 10 DCARP of each configuration is presented in Figure 9. For each instance, all found local optima were used to calculate the FDC in our analysis.

\subsubsection{Auto-correlation}
The auto-correlation measures the local ruggedness of the fitness landscape based on random-walk sampling \cite{weinberger1990correlated,tong2022makes}. It calculates the expected correlation between the first $T-\tau$ and last $T-\tau$ subsequences of a fitness sequence $\left\{c_{1}, c 2, \ldots, c_{T}\right\}$ corresponding to the solutions obtained by the random walk. The auto-correlation is estimated according to:

$$
R(\tau)=\frac{\sum_{t=1}^{T-\tau}\left(c_{t}-\bar{c}\right)\left(c_{t+\tau}-\bar{c}\right)}{\sum_{t=1}^{T}\left(c_{t}-\bar{c}\right)}
$$

where $\bar{c}$ is the mean fitness of the whole sequence. 


==> methodology-old.tex <==
\section{Methodology}
\label{sec:methodology}


\subsection{Dataset Selection}


In our empirical study, we follow the criteria below to select the datasets for investigation:

\begin{itemize}
    \item To improve the reproducibility of the experiment, we selected datasets that are publicly available.
    \item To mitigate bias, the datasets come from diverse domains
    \item The dataset should have been used by more than one peer-reviewed papers, and hence we rule out less reliable data.
    \item We also need to ensure that the dataset is free of missing values and repeated entries. 
\end{itemize}

According to the above, we selected 12 datasets, as shown in Table.

\subsection{Context Settings}

\subsection{Test Generators}

To

\subsection{Metrics}


\subsection{Protocol}



\subsection{Dataset}
We describe 12 popular public datasets for fairness testing as follows:
\begin{itemize}
        \item Adult Dataset: The Adult Dataset\cite{adultdataset2017} is a commonly used dataset in machine learning and data mining for predicting whether an individual's annual income exceeds 50,000. It contains individual attributes extracted from U.S. Census data, including age, work category, education level, marital status, occupation, and more.
    \item German Credit Dataset: The German Credit dataset\cite{germancreditdataset1994} consists of 1,000 instances that classify individuals based on credit risk using 20 attributes. The dataset includes four protected attributes: age, sex, foreign worker status, and personal status.
    \item Dutch Census Dataset: The Dutch Census dataset\cite{defaultcreditdataset2016} is based on population census data from the Netherlands, detailing information like occupation, education, and employment. The exact number of instances, features, and protected attributes may vary depending on the version of the dataset.
    \item Bank Marketing Dataset: The Bank Marketing dataset\cite{bankdataset2014} is composed of 45,211 instances from a Portuguese banking institution’s direct marketing campaign. It contains 17 features, with age being the protected attribute.
    \item Credit Card Clients Dataset: The Credit Card Clients data-set\cite{defaultcreditdataset2016} is based on credit card payment information of clients in Taiwan from April 2005 to September 2005. It provides 23 features, with three protected attributes: sex, age, and marital status.
    \item COMPAS Dataset: The COMPAS dataset\cite{compasdataset2016} is a tool used within the US criminal justice system for assessing recidivism risk. It includes several features and protected attributes, notably race, sex, and age.
    \item Communities and Crime Dataset: The Communities and Crime dataset\cite{UCICommunitiesCrime1990} contains socio-economic and crime data of 1,994 US communities from 1994. It has 128 features, with the protected attributes being the racial and ethnic demographics.
    \item Diabetes Dataset: The Diabetes dataset \cite{mepdataset2015} contains diagnostic measurements from the National Institute of Diabetes and Digestive and Kidney Diseases. It includes features such as number of pregnancies, BMI, insulin level, and age, the last of which is the protected attribute.
    \item Ricci Dataset: The Ricci dataset\cite{ribeiro2016trust} is compiled from a US Supreme Court case and includes data related to job performance and promotion. The dataset contains various features, with race being the protected attribute.
    \item Student Dataset: The Student dataset\cite{studentperformancedataset2014} includes data about student achievements in secondary education of two Portuguese schools. It offers several features, with age and sex being the protected attributes.
    \item OULAD Dataset: The OULAD dataset\cite{homecreditdataset2017} contains information about students' learning activities in online courses provided by the Open University. It provides multiple features, with age and gender being the protected attributes.
    \item Law School Dataset: The Law School dataset \cite{hearthealthdataset2001} includes data from law schools in the United States, such as LSAT scores, undergraduate GPA, and law school grade point averages. It has several features, with race, sex, and age being the protected attributes.
\end{itemize}

\subsection{Test Generation Method}

There are various test generation methods used in individual fairness testing to identify discriminatory behavior and improve the fairness of machine learning models. we use three specific test generation methods: ADF, AEQUITAS, and EIDIG.
\begin{itemize}
    \item AEQUITAS\cite{galhotra2017fairness}: It is a method designed to locate instances of individual discrimination in a given dataset. Its approach consists of two phases: a global phase and a local phase. The global phase involves a random search through the dataset, while the local phase employs a more targeted, directed search. In guiding the local phase, AEQUITAS offers three schemes: random, semi-directed, and fully-directed. The fully-directed scheme is typically the most effective as it leverages specific information about the dataset to direct the search for discriminatory instances. However, the choice between the three schemes can be adjusted based on the specifics of the dataset and the resources available for the search.
    \item ADF\cite{zhang2021fairness}: It is a test generation method that aims to identify and mitigate biases in machine learning models by generating adversarial examples. It operates by constructing input samples that are intentionally designed to expose discriminatory behavior in the model. ADF utilizes gradient information extracted from the white-box DNN model to guide the generation process. By perturbing the input features based on the model's gradients, ADF generates adversarial examples that highlight potential biases. These examples are then used to expand the training dataset and retrain the model, aiming to improve fairness.
    \item EIDIG\cite{zheng2022neuronfair}: It is a test generation method that employs an evolutionary algorithm to generate discriminatory samples. It starts by constructing an initial population of input samples. These samples are evaluated based on their discriminatory potential using fairness metrics or a fairness oracle. The algorithm then applies genetic operators such as mutation and crossover to evolve the population and generate new discriminatory samples. EIDIG improves the discriminatory nature of the samples by selecting and evolving the fittest individuals. The generated discriminatory samples can be used for fairness evaluation and model improvement.
\end{itemize}

\subsection{Experiment Design}

Deep Neural Networks (DNNs) are a powerful class of machine learning models that have demonstrated extraordinary performance in various complex tasks, such as image recognition, natural language processing, and even complex games. However, despite their robust performance, they are not immune to the influences of their training conditions or 'contexts', which include hyperparameters, labels, and selection bias.

Hyperparameters in DNNs, such as learning rate, regularization parameters, or the architecture of the network itself, govern the model's learning process and thus heavily influence its performance and behavior. The labels provided during supervised learning determine the patterns and relationships the model learns to recognize. Meanwhile, selection bias in the training data can lead to skewed or biased learning, leading to biases in the DNN's predictions. Each of these contexts can have significant impacts on the DNN's behaviors and, consequently, the outcomes of model testing.

In the arena of fairness testing, the significance of these contexts takes on an even greater role. Any biases present in labels or data selection can propagate through the DNN's complex layers, leading to discriminatory predictions. Similarly, hyperparameters, despite primarily being tuned for performance optimization, can inadvertently influence the fairness of the DNN. Hence, understanding the interplay between these contexts and their impact on fairness testing in DNNs is crucial for the development of ethically sound AI systems.

\subsubsection{RQ1:which context (hyperparmeter/label/selection) is the most influential on Fairness Testing?}
The impact of context on DNN fairness can be considered by drawing analogies to software testing. For instance, a DNN model with its configuration can be compared to a software program and its settings. The training data used for a DNN equates to the initial test suite in software testing, while the adjustment of hyperparameters, labels, and selection strategies aligns with the generation of additional software tests. Improvements in DNN fairness through context adjustment can be likened to software improvements following bug fixes.
To investigate the influence of context on DNN fairness, we suggest the following experimental design:

Experiment Design: We start with a DNN model, denoted as $M_0$, and define a set of contexts that consist of various combinations of hyperparameters, labels, and input selection methods. For each context, we train $M_0$ and evaluate the resulting model fairness.For instance, we generate a range of values for hyperparameters and use different label configurations and selection strategies to mirror a diversity of real-world scenarios. This diversity is analogous to the generation of different software tests.We then train the DNN model under each context, yielding a series of models $M_1, M_2, \ldots, M_n$, where each model corresponds to a specific context. This process mirrors the iterative aspect of software testing and fixing bugs.Finally, we measure the fairness of each model $M_i$ using adequacy metrics and fairness metrics, such as LSA,DSA,NC,NBC,SNAC and individual fairness. By analyzing these adequacy and fairness measures in relation to the contexts used, we can determine which contexts are the most influential in establishing DNN fairness.
Ideally, we would expect to uncover certain contexts that consistently lead to improved fairness, signifying their substantial role in ensuring DNN fairness.
\subsubsection{RQ2:How are correlation between adequacy and fairness metric under changing context?}
In the realm of fairness testing for Deep Neural Networks (DNNs), the correlation between adequacy(the measure of how well a model has been tested )and fairness metrics can offer valuable insights into the effectiveness of the testing process. However, the interplay between these measures can be significantly influenced by the context in which the model is trained and tested, including the hyperparameters, the provided labels, and the selection bias in the training data\cite{zhang2023rethinking,zheng2022neuronfair,karkkainen2021fairface}.
there may exist a complex relationship among different DNN test adequacy and fairness metrics under varying contexts. Understanding these relationships is crucial in making informed choices during the testing process, such as deciding which fairness metric to prioritize given the context or how to adjust hyperparameters to optimize both adequacy and fairness.In this research question, we aim to uncover the correlation or even partial ordering among adequacy and fairness metrics under varying contexts in fairness testing.

Experiment Design:To investigate this research question, we derive a range of values for each adequacy indicator and fairness criterion according to RQ1. For example, for neuron coverage (NC), we might obtain a sequence of values $N C_{F}=\left(N C_{0}^{F}, N C_{1}^{F}, \ldots, N C_{n}^{F}\right)$ where $n$ is the total number of input samples introduced set.Following this, we perform a correlation analysis on the collected data as well as the computed fairness metrics to discern whether there are strong correlations or partial orders among these metrics in different contexts. This analysis will shed light on how the changing environment in fairness testing affects the interplay between test adequacy and fairness, thereby guiding the development of more efficient and fair DNN models.
\subsubsection{RQ3: How context changes the test adequacy landscape using landscape analysis?}
The adequacy and fairness of DNNs can be profoundly impacted by different contextual factors, including hyperparameters, labels, and selection biases. These elements shape the testing landscape, affecting the test adequacy - a measure of how comprehensively the model has been tested. A critical question in fairness testing research is understanding how changes in context alter the test adequacy landscape. This understanding can guide the design of more effective testing strategies and contribute to improving the fairness of DNNs.
In this research question, we aim to perform a landscape analysis to investigate how changes in context  influence the test adequacy landscape in fairness testing.

Experiment Design: To address this research question, we take a given DNN model F and systematically modify the contextual factors - adjusting hyperparameters, changing labels, and introducing different degrees of selection bias. For each modified context, we evaluate the test adequacy of the model using various metrics such as Neuron Coverage (NC), Neuron Boundary Coverage (NBC), and others.
We then represent each modified context along with its corresponding test adequacy metrics in a multidimensional landscape. By analyzing this landscape, we can observe how changes in context alter the test adequacy landscape - that is, how the test adequacy of model F changes under different contexts. We can further identify certain patterns or trends in the landscape, such as regions of the context space that consistently lead to higher or lower test adequacy.
This landscape analysis provides valuable insights into the relationship between context and test adequacy in DNNs, contributing to our understanding of how to navigate the complex testing landscape effectively. These findings can guide the selection of appropriate contexts in DNN testing to ensure both high test adequacy and fairness.



%\subsubsection{Analysis}

==> renew.tex <==







Why not consider feature bias？
Feature bias refers to the unbalanced distribution of different features in the data or in relation to sensitive attributes (e.g., race, gender, age, etc.). Although feature bias may affect model training and prediction results, most papers usually focus more on label bias and select bias than feature bias when considering model fairness.
The reason is followed as:
\begin{itemize}
    \item Label bias and selection bias are directly related to the predictive results of the model as they are related to data labelling and sample selection.
    \item Individual fairness is concerned with whether similar individuals obtain similar predictions. Group fairness is concerned with whether the model's predictions are equal across groups. They are both directly related to the predictions.
    \item For feature bias, dealing with feature bias requires measures at the data preprocessing stage, such as feature importance selection, data sampling, or data augmentation.In pratice, dealing with feature bias is often very complex. On the other hand,Label bias and selection bias are only related to the distribution and labelling of the data samples themselves, which are easy to identify and handle.
\end{itemize}

why choose hp?
\begin{itemize}
    \item Hyperparameters directly affect model performance and prediction quality~\cite{chakraborty2020fairway,tizpaz2022fairness,zafar2017fairness}.
    \item Tuning hyperparameters is a relatively flexible and efficient method that can be achieved by simple techniques such as cross-validation, grid search or Bayesian optimisation.
    \item Hyperparameters are universal to different datasets.
\end{itemize}





Hyperparameter Hypothesis:
The choice of hyperparameters should not significantly affect the fairness of the model. That is, the performance of the model in terms of fairness should be consistent even for different hyperparameter settings~\cite{chakraborty2019software,chakraborty2020making,gohar2023towards,tizpaz2022fairness}.
Label Bias:
Assuming that the labels of the training data are independent of subgroups, the labels do not systematically bias the prediction results for specific subgroups. This prevents the labels themselves from carrying unfair information~\cite{zhang2021ignorance,chakraborty2021bias,chakraborty2022fairssl,chakraborty2020fairway,chen2021understanding}.

Select Bias:
Selection bias has been reasonably tackled or rectified and will not significantly affect the results of the fairness test~\cite{chen2022maat,chakraborty2020fairway,chakraborty2021bias,karkkainen2021fairface,mambreyan2022dataset}.


Fairness issue/bug:
A fairness bug in a software system refers to any flaw or imperfection that leads to a misalignment between the actual fairness conditions and the desired fairness conditions set by the developers. The specific fairness conditions that need to be achieved depend on the fairness definition adopted for the particular software or machine learning model being tested.The imperfections can manifest as unfair predictions that violate individual fairness or discrepancies in outcomes among different demographic groups that surpass a predetermined threshold for group fairness. ~\cite{finkelstein2008fairness,chakraborty2020making,chen2021fairness}

% violate individual fairness:
% Individual fairness refers to the idea that similar individuals should receive similar treatment or predictions from the software system. A fairness bug could occur when the system produces unfair predictions that treat similar individuals differently, leading to discrepancies in their treatment based on certain sensitive attributes (e.g., race, gender, etc.).

% Group Fairness Discrepancies:
% Group fairness focuses on the overall fairness of outcomes between different population groups. Fairness deficits may occur if there are significant differences in outcomes between groups that exceed predefined thresholds or violate developer-defined fairness criteria.























\section{}

Why did we choose these 3 types of test contexts?
In our empirical study, we conducted a preliminary study of 48 articles and found that the main focus in current fairness testing is on the classification problem. The classification problems are usually based on sets of data. And the data are historical data sets, which has a tendency to bias. And there are two main sources of this bias: label bias (inaccurate labeling) and select bias (inappropriate selection).

On the other hand, since machine learning algorithms may be encoded as processing, decision logic, and runtime configurations. Each part of the algorithm may introduce fairness problems in the final software system. In deep neural networks, especially hyperparameter configurations, the neural network will generate neural networks with completely different structures depending on the hyperparameter configurations, and thus it may introduce a fairness bias.

\subsection{dataset selection}
In our empirical study, we used the following criteria to select datasets.
\begin{itemize}
    \item to improve the reproducibility of the experiment, we selected datasets from public databases.
    \item to enrich the diversity of potential experimental findings, we selected datasets from different domains.
    \item to ensure the robustness of experimental data in the future. The datasets we adopt are widely used and tested in the literature in a large number of fairness testing domains.
\end{itemize}
Based on the above criteria, we have listed 12 publicly available datasets, and the characteristics of each dataset are summarised in the table below:
\begin{table}
\caption{The real world  fairness dataset.}
\label{tb:fdt}
\begin{tabular}{c|c|c|c|c|c}
\toprule
    \textbf{Dataset} & \textbf{Class} &\textbf{Class ratio(+:-)}& \textbf{Domain} & \textbf{Size} & \textbf{Sensitive Attibutes}\\
    \midrule
    \textsc{Adult}& Binary&$1:3.03$ & Finance&$ 45222$& Sex, Race, Age\\
    \midrule
    \textsc{Bank}& Binary &$1:7.55$& Finance&$ 45211$& Age,Marital\\
    \midrule
    \textsc{German}& Binary &$2.33:1$& Finance&$ 1000$& Sex,Age\\
    \midrule
    \textsc{Credit}& Binary &$1:3.52$& Finance&$ 30000$& Sex,Marital,Education\\
    \midrule
    \textsc{Compas}& Binary &$1:1.20$& Criminology&$ 6172$& Sex,Race\\
    \midrule
    \textsc{Law School}& Binary &$8.07:1$& Education&$ 20708$& Sex,Race\\
    \midrule
    \textsc{Student}& Binary &$1:2.40$& Education&$ 648$& Sex,Age\\
    \midrule
    \textsc{Communities and Crime}& Multi &$-$& Criminology&$ 2215$& Race,Age\\
    \midrule
    \textsc{KDD Census-Income}& Binary &$1:15.30$& Criminology&$ 284556$& Sex,Race\\
    \midrule
    \textsc{Dutch}& Binary &$1:1.10$& Finance&$ 60420$& Sex\\
    \midrule
    \textsc{Diabetes}& Binary &$1:3.13$& Healthcare&$ 45715$& Race\\
    \midrule
    \textsc{OULAD}& Multi &$-$& Education&$ 21562$& Race\\
\end{tabular}
\end{table}

why choose these three Test generation methods?
In the field of fairness testing, test input generation automatically generates valid samples that may lead to bias, thus revealing the fairness of a software system. A large number of approaches to fairness test generation have been mentioned in recent years. For example, THEMIS, AEQUITAS, SG, ADF, ExpGA, SFBT and EIDIG, etc.
In this empirical study, we select the test generation method by following 4 criteria:
\begin{itemize}
    \item the method is applicable to DNN models and can guide the generation of individual discrimination sample instances.
    \item the method is state-of-the-art.
    \item the method is public or code examples can be found.
    \item the method can use test the individual fairness.
\end{itemize}


In addition, for different test input generation methods, we would like to possibly keep the algorithms in the methods consistent so as to avoid unnecessary interference. We selected AEQUITAS, ADF and EIDIG according to the above criteria. 

These three methods all use two-phase search algorithms to find instances of individual discrimination. The two-phase search is mainly global search and local search. In the global search phase, the test method is guided by the gradient to find possible instances of bias close to the decision boundary by progressively perturbing the inputs; in the local search phase, the test method will be further guided by the gradient to search the neighbourhoods of the single instances of bias that have already been found in order to find more instances of bias.

why choose this five adequacy metric and Individual Fairness metric?
As our goal is to investigate the relevance of adequacy metric and fairness metric on testing DNNs. We conducted a comprehensive survey of existing adequacy metrics used to evaluate test DNNs.
A set of testing coverage metrics of models as shown in the following table.
\begin{table}[Test coverage metrics]
    \centering
    \begin{tabular}{c|c}
         &  \textbf{Metric Name} & \textbf{Description}\\
         & NC & Neuron Coverage\\
         & KNC & K-multisection Neuron Coverage\\
         & SNAC & Strong Neuron Activation Coverage\\
         & NBC & Neuron Boundary Coverage\\
         & TKNC & Top-k Dominant Neuron Coverage\\
         & TKNP & Top-k Dominant Neuron Patterns Coverage\\
         & LSA & Surprise adequacy \\
         & DSA & Surprise adequacy \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
In our review of 41 academic papers on deep neural network test generation over the past five years, we found that the vast majority of studies utilized the Neuron Coverage (NC), Neuron Boundary Coverage (NBC), and Strong Neuron Activation Coverage (SNAC) metrics to measure test sufficiency. These metrics are widely accepted and applied in DNN and ML test generation research, aiding in evaluating model performance during testing and effectively identifying potential weaknesses and deficiencies. This finding reflects the dominant position of NC, NBC, and SNAC in assessing test adequacy, as they have become key standards for evaluating DNN and ML model test generation.Furthermore, we noticed that 15 papers mentioned the surprise adequacy metric proposed by Kim et al., including Likelihood-based Surprise Adequacy (LSA) and Distance-based Surprise Adequacy (DSA).
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  Metric Name & Times \\
         & NC & 41\\
         & KNC & 38\\
         & SNAC & 41\\
         & NBC & 41\\
         & TKNC & 30\\
         & TKNP & 30\\
         & LSA & 15 \\
         & DSA & 15 \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
{\color{red} Regarding the six metrics associated with Coverage, the definitions for Neuron Coverage (NC), K-Neuron Coverage (KNC), Top-k Neuron Coverage (TNKC), and Top-k Neuron Patterns (TNKP) share substantial similarities. Nonetheless, NC stands out as the most favored and prevalently used, which prompts us to primarily lean towards it. Contrastingly, Strong Neuron Activation Coverage (SNAC) and Neuron Boundary Coverage (NBC) are beneficial enhancements to NC, effectively addressing the coverage of boundary areas that NC might overlook, hence rendering the coverage assessment more exhaustive and insightful. As for the domain of surprise adequacy, currently, the only metrics available are Likelihood-based Surprise Adequacy (LSA) and Distance-based Surprise Adequacy (DSA), both of which we decided to include in our study. Consequently, in light of the aforementioned factors, we have opted for these five metrics as a means of evaluating the adequacy of our testing procedures.}


On the extensive literature in the field of test DNN systems, for adequacy metrics, there are metrics that describe the behaviour of the neurons based mainly on the output values of the neurons determined from the training data, among which the commonly used metrics are NC,NBC,SNAC. In addition, for the training data, there are also the DSA and LSA based Surprise adequacy metrics.

Likelihood-based Surprise adequacy (LSA) assesses the relative novelty (i.e., surprise) of a given new input with respect to the inputs used for training by measuring the probability density of each activation value across all activated neurons.

Distance-based Surprise adequacy (DSA) assesses the relative novelty (i.e., surprise) of a given new input with respect to the input used for training by measuring the Euclidean distance between the activated neurons of the new input and the activated neurons of the training input.

NC：Neuron coverage is the ratio of the number of neurons activated in the test input to the total number of neurons in the DNN.

NBC：The neuron boundary coverage is primarily measured the region of edge cases (upper and lower boundary values) covered in a given input set $T$.It is defined as the ratio of the number of edge cases covered to the total number of edge cases ($2 × |N|$).

SNAC:Strong Neuron Activation Coverage is similar with NBC. it is measured the region of edge cases(higher upper boundary) covered in a given input set $T$.It is defined as the ratio of the number of edge cases on the coverage to the total number of edge cases ($|N|$).

IDI：
In software testing, we need to consider the fairness of the model, which means that we cannot allow the model to make discriminatory judgements or produce different predictions because of particular attributes such as race, gender, age or disability. However, most of the existing metrics for assessing fairness are focused on group fairness, but we cannot ignore individual fairness, especially when dealing with individuals with similar characteristics, and need to ensure that decisions are consistent.
In general, we think of individual fairness as similar individuals whose predictions remain consistent, but the reason for this definition is mainly the comparison with the nearest neighbouring point. A new measure of individual fairness is introduced by Chakrabortyet al. They measure the proportion of the population whose predictions are reversed (e.g., from acceptance to rejection) when the predictions are reversed.

Based on this definition, we primarily consider situations in which model outputs change when we change some of the protected characteristics in an instance while holding all other non-protected characteristics constant. We call instances that produce such changes individual discrimination instances. Thus, we can judge whether the model is fair by measuring the proportion of individual discrimination instances that the model produces ($individual discrimination instances/total sample instances$).


how to select different contexts ?
the setting of the Hyperparameter configurations considered in our experiments
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
         &  \textbf{Name}&  \textbf{Description}&  \textbf{Range}\\
         &  Learning rate & &$R[10^{-1}-10^{-6}]$\\
         &  Batch size& &$ 2^{n},n = R[4,10]$\\
         &  Number of epochs& &$R[50-200]$\\
         &  Number of neurons& &$ 2^{n},n = R[4,10]$\\
         &  Activation function& & ReLU, Sigmoid, Tah\\
         &  Optimizer& &Adam, SGD\\
         &  Number of layers& &$Z[2-10]$\\
         &  Regularization& &$R[10^{-1}-10^{-5}]$\\
         &  weight method& &Random, xavier, he\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

label Bias:
When discussing label bias, we first need to understand that in each dataset used for training a machine learning model, the proportion of different labels can vary widely. These proportions can either mirror the actual distribution of classes in the problem space or they can be artificially adjusted to meet specific training objectives or to address class imbalance.

To investigate the influence of  label biases on model fairness, we intentionally adjust the proportion of each label within the dataset. Furthermore, we also combine the ratios of different labels within each dataset, keeping them within certain constraints. Thus, we are able to delve into the impact of label bias on the model from multiple angles.

Our experimental framework involves modifying the distribution of labels across different datasets, which allows us to study the model's response to different labeling scenarios and evaluate how various types of label biases can influence model fairness and performance. We also experiment with combining different label proportions, giving us a better understanding of how mixed labeling biases might impact model behavior.
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \textbf{Dataset} &\textbf{Range of Class ratio}\\
         & 
    \textsc{Adult}&${1-5}:{1-5}$ \\
    \midrule
    \textsc{Bank} &${1-8}:{1-8}$\\
    \midrule
    \textsc{German} &${1-3}:{1-3}$\\
    \midrule
    \textsc{Credit} &${1-4}:{1-4}$\\
    \midrule
    \textsc{Compas} &${1-3}:{1-3}$\\
    \midrule
    \textsc{Law School}&${1-10}:{1-10}$\\
    \midrule
    \textsc{Student} &${1-4}:{1-4}$\\
    \midrule
    \textsc{Communities and Crime} &${1-4}:{1-4}$\\
    \midrule
    \textsc{KDD Census-Income} &${1-20}:{1-20}$\\
    \midrule
    \textsc{Dutch} &${1-4}:{1-4}$\\
    \midrule
    \textsc{Diabetes} &${1-4}:{1-4}$\\
    \midrule
    \textsc{OULAD} &${1-4}:{1-4}$\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

select bias: 
Within each fairness dataset, the ratio of sensitive attributes varies. In order to investigate the influence of various select biases on model fairness, we intentionally adjust the proportion of each protective attribute within each dataset, based on fairness learning. Moreover, we combine the ratio of different sensitive attributes within each dataset, constrained within a certain range. As a result, we delve into the effects of select bias on fairness from a multitude of perspectives.

By manually scaling the ratio of sensitive attributes, we can simulate a range of potential bias environments, a critical step in understanding how these biases can impact model fairness. We have established an experimental framework. we experiment with combinations of different sensitive attribute ratios to assess the impact of mixed bias compositions on model fairness. By mixing the ratios of different sensitive attributes within a certain range, we can gain a better understanding of how these biases interact and influence the fairness of the model. For instance, bias for certain sensitive attributes might augment or neutralize the bias for other attributes, while in other cases, these biases might operate in conjunction to create larger issues of fairness.

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \textbf{Dataset}&\textbf{sensitive attribute} &\textbf{Range of sensitive attribute ratio()}\\
         & 
    \textsc{Adult}& Sex, Race, Age&${{10-90}:{10-90}}$,${{10-90}:{10-90}}$, ${{10-90}:{10-90}}$ \\
    \midrule
    \textsc{Bank}&Age, Marital &${{10-90}:{10-90}}$, ${{10-90}:{10-90}}$\\
    \midrule
    \textsc{German}& Sex, Age &${{10-90}:{10-90}}$, ${{10-90}:{10-90}}$\\
    \midrule
    \textsc{Credit}& Sex, Marital, Education &${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$, ${{10-90}:{10:90}:{10:90}}$\\
    \midrule
    \textsc{Compas}& Sex, Race &${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$\\
    \midrule
    \textsc{Law School}& Sex, Race&${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$\\
    \midrule
    \textsc{Student}& Sex, Age &${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$\\
    \midrule
    \textsc{Communities and Crime}& Race, Age &${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$\\
    \midrule
    \textsc{KDD Census-Income}& Sex, Race &${{10-90}:{10:90}}$, ${{10-90}:{10:90}}$\\
    \midrule
    \textsc{Dutch}& Sex &${{10-90}:{10:90}}$\\
    \midrule
    \textsc{Diabetes}& Race &${{10-90}:{10:90}}$\\
    \midrule
    \textsc{OULAD}& Race&${{10-90}:{10:90}}$\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
discussion

==> results_old.tex <==
%adequency
%HP-Bank-<0.05/>=0.05: 7/8
%HP-Adult-<0.05/>=0.05:9/6
%HP-Greman-<0.05/>=0.05:7/8
%HP-Credit-<0.05/>=0.05:9/6
%HP-Compas-<0.05/>=0.05:9/6
%HP-Lawschool-<0.05/>=0.05:9/6
%HP-Student-<0.05/>=0.05:9/6
%HP-Crime-<0.05/>=0.05:9/6
%HP-KDD-<0.05/>=0.05:8/7
%HP-Dutch-<0.05/>=0.05:9/6
%HP-Diabete-<0.05/>=0.05:9/6
%HP-Oulad-<0.05/>=0.05:9/6

%SB-Bank-<0.05/>=0.05: 10/5
%SB-Adult-<0.05/>=0.05:8/7
%SB-Greman-<0.05/>=0.05:11/4
%SB-Credit-<0.05/>=0.05:11/4
%SB-Compas-<0.05/>=0.05:12/3
%SB-Lawschool-<0.05/>=0.05:12/3
%SB-Student-<0.05/>=0.05:11/4
%SB-Crime-<0.05/>=0.05:10/5
%SB-KDD-<0.05/>=0.05:13/2
%SB-Dutch-<0.05/>=0.05:11/4
%SB-Diabete-<0.05/>=0.05:12/3
%SB-Oulad-<0.05/>=0.05:13/2

%LB-Bank-<0.05/>=0.05: 9/6
%LB-Adult-<0.05/>=0.05:10/5
%LB-Greman-<0.05/>=0.05:9/6
%LB-Credit-<0.05/>=0.05:8/7
%LB-Compas-<0.05/>=0.05:9/6
%LB-Lawschool-<0.05/>=0.05:9/6
%LB-Student-<0.05/>=0.05:9/6
%LB-Crime-<0.05/>=0.05:10/5
%LB-KDD-<0.05/>=0.05:9/6
%LB-Dutch-<0.05/>=0.05:9/6
%LB-Diabete-<0.05/>=0.05:7/8
%LB-Oulad-<0.05/>=0.05:9/6
%fairness
%HP-Bank-<0.05/>=0.05: 0/15
%HP-Adult-<0.05/>=0.05:1/14
%HP-Greman-<0.05/>=0.05:0/15
%HP-Credit-<0.05/>=0.05:1/14
%HP-Compas-<0.05/>=0.05:2/13
%HP-Lawschool-<0.05/>=0.05:0/15
%HP-Student-<0.05/>=0.05:0/15
%HP-Crime-<0.05/>=0.05:1/14
%HP-KDD-<0.05/>=0.05:0/15
%HP-Dutch-<0.05/>=0.05:2/13
%HP-Diabete-<0.05/>=0.05:0/15
%HP-Oulad-<0.05/>=0.05:0/15

%SB-Bank-<0.05/>=0.05: 4/11
%SB-Adult-<0.05/>=0.05:5/10
%SB-Greman-<0.05/>=0.05:6/9
%SB-Credit-<0.05/>=0.05:4/11
%SB-Compas-<0.05/>=0.05:8/7
%SB-Lawschool-<0.05/>=0.05:9/6
%SB-Student-<0.05/>=0.05:2/13
%SB-Crime-<0.05/>=0.05:1/14
%SB-KDD-<0.05/>=0.05:5/10
%SB-Dutch-<0.05/>=0.05:3/12
%SB-Diabete-<0.05/>=0.05:2/13
%SB-Oulad-<0.05/>=0.05:2/13

%LB-Bank-<0.05/>=0.05: 1/14
%LB-Adult-<0.05/>=0.05:2/13
%LB-Greman-<0.05/>=0.05:2/13
%LB-Credit-<0.05/>=0.05:4/11
%LB-Compas-<0.05/>=0.05:2/13
%LB-Lawschool-<0.05/>=0.05:1/14
%LB-Student-<0.05/>=0.05:2/13
%LB-Crime-<0.05/>=0.05:0/15
%LB-KDD-<0.05/>=0.05:3/12
%LB-Dutch-<0.05/>=0.05:3/12
%LB-Diabete-<0.05/>=0.05:4/11
%LB-Oulad-<0.05/>=0.05:3/12

%FDC


%correlation length


\section{Study Results}
\label{sec:evaluation}

In this section, we illustrate and discuss the results of our study.


\subsection{Variability by Context Settings (RQ$_2$)}

\subsubsection{Method}

To understand RQ$_2$, in each context/dataset, we calculate the  coefficient of variation (CV) for data under different context settings over all combinations of the generators and metrics. CV is a scale-/unit-free metric that has been commonly used in software engineering to measure variability [].
%, i.e., the ratio $\mu \over \sigma$ between standard deviation $\sigma$ and mean $\mu$. 

Specifically, since we have 3 generators and 5 metrics, we record the individual CV for every $15$ case under each context type and dataset, i.e. ${{\mu_i} \over {\sigma_i}}\times 100\%$, where $\mu_i$ and $\sigma_i$ are the mean and standard deviation on the average metric values (over 30 runs) of 10 context settings in the $i$th case, respectively. In particular, the literature often uses $5\%$ as an indication threshold of whether the variability is significant for software engineering problems []. That is, if we observe $CV>5\%$ then there is likely to be a substantial fluctuation. As such, we aim to examine whether the changing context settings would considerably affect the testing results.

\subsubsection{Result}

The results are plotted in Figure where we count the number of cases with $CV\leq5\%$ and otherwise within the 15 generator-metric combinations. As can be seen, for the adequacy metrics, there is only a moderate amount of cases where we observed $CV>5\%$ for all context types (6-8 for hyperparameter; 2-5 for selection bias; and 6-8 for label bias out of 15), suggesting that varying context settings may not create significant implications for the results. 

Conversely, for the fairness metric, we see that in general, the context change would often have a large effect that leads to results with substantial variability, i.e., the number of cases with $CV>5\%$ out of 15 can be 13-15 for hyperparameter; 6-14 for selection bias; and 11-14 for label bias. In many cases, the CV would \textcolor{red}{reach \%}. Particularly, changing hyperparameters alone can lead to the most significant changes to fairness testing results in the majority of the datasets. 

From the above, we observe a rather significant discrepancy between the CV for the test adequacy metric and that for the fairness metric. This suggests some complex and non-linear relationships between the two metric types, which we will further explore in Section [].

%As a result, we say:

\begin{quotetitlebox}{\textbf{Summary of Findings for RQ$_2$}}
   \noindent
   Within each context type, changing settings may not have a significant impact on the adequacy results, but it leads to much more substantial variability in terms of fairness metric, particularly when varying hyperparameter settings.
\end{quotetitlebox}
%count the number CV < 5%, [5,50],[50,100],[100->] CV as a baseline by Patterns in the Chaos—A Study of Performance Variation and Predictability in Public IaaS Clouds
%White-Box Performance-Influence Models:A Profiling and Learning Approach
%A Framework for the Automatic Execution of Measurement-based Experiments on Android Devices
%Twins or false friends? A study on energy consumption and performance of configurable software
%Analyzing the impact of workloads on modeling the performance of configurable software systems

%Do contexts have an impact? (CV for variability with counts under different intervals)
%Do contexts contribute to the same influence?

\input{Table/rq1-new}

\subsection{Implication to Quality Metrics (RQ$_1$)}



\subsubsection{Method}

To study RQ$_1$, we consider test adequacy and fairness metrics independently. In particular, for each context type, we summarized the mean results across all five test adequacy metrics and their corresponding fairness metrics, each with 10 context settings and 30 repeated runs, on a generator-dataset case, giving us $10\times30=300$ data points for each metric in a case. Since there are three generators and 12 datasets, we are comparing the implication of the three context types over $3\times12=36$ cases. We also compare with a baseline that comes with optimized hyperparameters for accuracy as used in previous work while without any selection and label bias; this helps us to understand if considering changes in a context type would alert the results compared with the case when none of the contexts is considered. To ensure statistical significance, we report on the mean rank computed by the Scott-Knott test over the five metrics. 

%TODO, move the baseline to genearl

\subsubsection{Results}

For test adequacy metrics, as shown in Table [], we see that testing with both the selection and label bias would have better ranks in general compared with the baseline, leading to 28 (78\%) and 33 (92\%) better cases out of 36, respectively. When ignoring the optimized Hyperparameter, in contrast, there are 28 (78\%) cases worse than the baseline. This means that non-optimized hyperparameters would create DNNs that are more difficult for the generators to reach better adequacy results while the presence of selection/label bias would often lead to easier-to-be-tested DNNs. 

%Indeed, among the three context types, testing on non-optimized hyperparameters often has the worst ranks for 28 out of 36 cases while testing with the selection and label bias is ranked the best over 15 and 21 cases, respectively. 


%From the standard error, we see that testing under hyperparameter leads to a larger deviation in the test adequacy in all cases. In contrast, testing under label bias generally tends to have the most stable results (28 out of 36 cases). 

From Table [], we compare the results on the fairness metric. Clearly, across all cases, testing under non-optimized hyperparameters leads to 14/36 (39\%) cases that exhibit more effective outcomes in finding fairness issues than the baseline. On the contrary, this number becomes 22 (61\%) and 20 (56\%) for testing under selection and label bias, respectively. 

Another pattern we found is that, for all context types, there is a moderate decrease in the performance deviation to baseline when compared with the case of test adequacy metrics, but the overall conclusion remains similar. This implies that a better adequacy metric value might not always lead to a better ability to find fairness issues. 

In summary, we conclude that:

%In particular, testing with both selection and label bias is ranked the best over 16 cases, but working on non-optimized hyperparameters only achieves the best rank for 9 cases.
 

%Yet, for fairness measurement, testing under different forms of selection bias has the most stable outcomes (29 out of 36 cases).


\begin{quotebox}
   \noindent
   \textbf{Summary} (RQ$_1$): Compared with the baseline of perfect assumption where none of the contexts exists, non-optimized hyperparameters often make significantly more challenging DNNs that cause the generators more struggle to improve test adequacy (78\%) and find fairness issues (61\%); while the presence of data bias generally leads to much easier DNNs that make the testing considerably more effective in terms of both metric types (56\%-92\%), particularly the label bias.
   

   %so that the diffcult DNN can stress the evaluation, and challenge papers that use the easy DNN
   %having bias get more fairness issue, hence testing more effective; this is just naive
\end{quotebox}


\begin{figure}[t]
     \centering
          \includegraphics[height=\columnwidth]{Figures/cv-count.pdf}         
     \caption{The number of cases with CV$\leq0.05$ and CV$>0.05$ over the 15 combinations of generators and metrics.}
    \label{fig:rq2}
\end{figure}

\subsection{Variability by Settings (RQ$_2$)}

\subsubsection{Method}

To understand RQ$_2$, in each context/dataset, we calculate the  coefficient of variation (CV) for data under different context settings over all combinations of the generators and metrics. CV is a scale-/unit-free metric that has been commonly used in software engineering to measure variability [].
%, i.e., the ratio $\mu \over \sigma$ between standard deviation $\sigma$ and mean $\mu$. 

Specifically, since we have 3 generators and 5 metrics, we record the individual CV for every $15$ case under each context type and dataset, i.e. ${{\mu_i} \over {\sigma_i}}\times 100\%$, where $\mu_i$ and $\sigma_i$ are the mean and standard deviation on the average metric values (over 30 runs) of 10 context settings in the $i$th case, respectively. In particular, the literature often uses $5\%$ as an indication threshold of whether the variability is significant for software engineering problems []. That is, if we observe $CV>5\%$ then there is likely to be a substantial fluctuation. As such, we aim to examine whether the changing context settings would considerably affect the testing results.

\subsubsection{Result}

The results are plotted in Figure where we count the number of cases with $CV\leq5\%$ and otherwise within the 15 generator-metric combinations. As can be seen, for the adequacy metrics, there is only a moderate amount of cases where we observed $CV>5\%$ for all context types (6-8 for hyperparameter; 2-5 for selection bias; and 6-8 for label bias out of 15), suggesting that varying context settings may not create significant implications for the results. 

Conversely, for the fairness metric, we see that in general, the context change would often have a large effect that leads to results with substantial variability, i.e., the number of cases with $CV>5\%$ out of 15 can be 13-15 for hyperparameter; 6-14 for selection bias; and 11-14 for label bias. In many cases, the CV would \textcolor{red}{reach \%}. Particularly, changing hyperparameters alone can lead to the most significant changes to fairness testing results in the majority of the datasets. 

From the above, we observe a rather significant discrepancy between the CV for the test adequacy metric and that for the fairness metric. This suggests some complex and non-linear relationships between the two metric types, which we will further explore in Section [].

As a result, we say:

\begin{quotebox}
   \noindent
   \textbf{Summary} (RQ$_2$): Changing context settings may not have a significant impact on the adequacy results, but it leads to much more substantial variability in terms of fairness metric, particularly when varying hyperparameter settings.
\end{quotebox}

\subsection{Correlation between Adequacy and Fairness (RQ$_3$)}


\subsection{Testing Landscape (RQ$_4$)}


\subsection{RQ1: Influence on different contexts}
% \subsubsection{Effect on adequacy metric}
% First, we investigated whether the values of the adequacy metrics changed significantly after changing different contexts based on the use of existing advanced test generation methods.
% \subsubsection{Effect on Fairness metric}
% Second, we investigated whether the value of the equity metric changed significantly after we used different contexts.
\subsubsection{method}
We analyze the changes in the values of the adequacy metrics due to different contexts, and present the results in Table RQ1. We note that after applying different contexts, among them the hyperparameter settings have the largest mean value and the smallest error on the adequacy metrics (i.e. DSA,LSA,NC, NBC, SNAC) tested on the 12 commonly used datasets. Our results suggest to the research community that hyperparameter settings have a significant impact on adequacy metrics.

To answer question 1, we use Latin hypercube sampling to take 10 times for each context task and then train the model in batches based on 12 different datasets and then sample generation in 3 different state-of-the-art test generation methods respectively. Thus we have a total of 3X10X12 = 360 applications. We performed 30 tests for each application. For each application, we calculated the difference in the mean of five adequacy metrics and the difference in one fairness metric. We then used the Scott-Knott test to investigate the variation in the values of the different metrics caused by different context tasks. In a nutshell, Scott-Knott sorts the list of treatments (adequacy metric of different contexts of different test generation method) by their median and SE. In table 1 , for each dataset of different test generation methods, we list the Scott-Knott ranking, median and error of the mean adequacy metric for different contexts and summarize the Scott-Knott ranking, median and error of the mean for all datasets.


%\input{Table/rq1-adq}
%\input{Table/rq1-fair}
\subsubsection{Results}

As illustrated in Table~\ref{tb:rq1}, we observe some interesting findings:
\begin{itemize}
    \item \textbf{Finding 1:} From Table~\ref{tb:rq1}, the hyperparameters were clearly more accurate than the label bias and select bias in all cases, as the former had the best Scott-Knott overall average score in all cases in the systems studied. Furthermore, we noticed that there were significant differences in the mean test adequacy metric across cases in different test generation methods. We observe a similar trend from the system in Table 1.

    \item \textbf{Finding 2:} For different dataset in Table~\ref{tb:rq1}, We observe that hyperparameters are best for affecting the adequacy and fairness of the test model.The same has also been registered in Table 2.
\end{itemize}


To conclude, we can answer \textbf{RQ1} as:


\begin{quotebox}
   \noindent
   \textit{\textbf{RQ1:} In general, hyperparameters tend to have the best influence on tests of adequacy and individual fairness.}
\end{quotebox}
\subsection{RQ2: Adequacy}
\subsubsection{method}
In this section, we present the results of 15 fairness-adequacy correlation measures, i.e., combining our fairness metric IDI and five adquacy metrics (DSA, LSA.) in three contexts (hyperaparameter, label bias and select bias). NC,NBC and SNAC) combined by computing Spearman's rank correlation coefficient. Foreach(fairness-adequacy metric pair) combination, we calculate the over all correlation between the 120 value differences of the two metrics.
We compare the correlation between adequacy metrics and fairness metrics in different contexts. The results provide insights for setting better conext in application scenarios where fairness is critical.

\begin{figure*}[t!]
\centering
     \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_1.pdf}
          \subcaption{Hyperparameter}
          \textit{($r=-0.14,p<0.01$)}
     \end{subfigure}
     ~
     \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_2.pdf}
          \subcaption{Label bias}
          \textit{(r=0.10,p=0.054)}
     \end{subfigure}
     ~
     \begin{subfigure}[t]{0.33\columnwidth}
          \centering
  % \includestandalone[width=\columnwidth]{Figures/rq2-1}
          \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_3.pdf}
          \subcaption{Selection bias}
          \textit{(r=0.58,p<0.01)}
     \end{subfigure}
\centering
     \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_4.pdf}
          \subcaption{Hyperparameter}
          \textit{(r=0.72,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_5.pdf}
        \subcaption{Label bias}
        \textit{(r=0.59,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_6.pdf}
         \subcaption{Selection bias}
         \textit{(r=0.35,p<0.01)}
    \end{subfigure}
\centering
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_7.pdf}
         \subcaption{Hyperparameter}
         \textit{(r=0.11,p=0.031)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_8.pdf}
         \subcaption{Label bias}
         \textit{(r=0.59,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_9.pdf}
         \subcaption{Selection bias}
         \textit{(r=-0.22,p<0.01)}
    \end{subfigure}
\centering
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_10.pdf}
         \subcaption{Hyperparameter}
         \textit{(r=-0.20,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_11.pdf}
         \subcaption{Label bias}
         \textit{(r=-0.85,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_12.pdf}
         \subcaption{Selection bias}
         \textit{(r=-0.66,p<0.01)}
    \end{subfigure}
\centering
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_13.pdf}
         \subcaption{Hyperparameter}
         \textit{(r=-0.05,p=0.39)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_14.pdf}
         \subcaption{Label bias}
         \textit{(r=-0.89,p<0.01)}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.33\columnwidth}
         \centering
         \includegraphics[width=\linewidth]{Figures/rq2_pdf/rq2_15.pdf}
         \subcaption{Selection bias}
         \textit{(r=-0.57,p<0.01)}
    \end{subfigure}
    \caption{RQ2, the correlation between a test adequacy metric and its fairness metric.}
    \label{fig:corr}
\end{figure*}



\begin{figure}[t!]
\centering
{
     \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/dsa-idi-hp.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.14, p<0.01$)}
     \end{subfigure}
     ~
        \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/dsa-idi-sb.pdf}
         \vspace{-0.6cm}
          \subcaption*{($r=0.58, p<0.01$)}
     \end{subfigure}
     ~
         \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/dsa-idi-lb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.10, p=0.054$)}
     \end{subfigure}
\subcaption{DSA-IDI}

    \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/lsa-idi-hp.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.72, p<0.01$)}
     \end{subfigure}
     ~
        \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/lsa-idi-sb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.35, p<0.01$)}
     \end{subfigure}
     ~
         \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/lsa-idi-lb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.59, p<0.01$)}
     \end{subfigure}
\subcaption{LSA-IDI}

    \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nc-idi-hp.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.11, p=0.031$)}
     \end{subfigure}
     ~
        \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nc-idi-sb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.22, p<0.01$)}
     \end{subfigure}
     ~
         \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nc-idi-lb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=0.59, p<0.01$)}
     \end{subfigure}
\subcaption{NC-IDI}

    \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nbc-idi-hp.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.20, p<0.01$)}
     \end{subfigure}
     ~
        \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nbc-idi-sb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.66, p<0.01$)}
     \end{subfigure}
     ~
         \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/nbc-idi-lb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.85, p<0.01$)}
     \end{subfigure}
\subcaption{NBC-IDI}


    \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/snac-idi-hp.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.05, p=0.39$)}
     \end{subfigure}
     ~
        \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/snac-idi-sb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.57, p<0.01$)}
     \end{subfigure}
     ~
         \begin{subfigure}[t]{0.33\columnwidth}
          \centering
          \includegraphics[width=\columnwidth]{Figures/correlation/snac-idi-lb.pdf}
          \vspace{-0.6cm}
          \subcaption*{($r=-0.89, p<0.01$)}
     \end{subfigure}
\subcaption{SNAC-IDI}
     }
    \caption{Spearman correlations (and their $p$ values) between adequacy and fairness by contexts.}
    \label{fig:sp}
\end{figure}

\subsubsection{Results}

With figure~\ref{fig:corr}, we can observe some patterns:
\begin{itemize}
    \item \textbf{Finding 3:} Overall, the 15 metric pairs in Figure 2, 5 showed significant positive correlations, 7 showed significant negative correlations, and 3 had no significant correlations. In addition, we found individual cases where different pairs of metrics did not show consistent correlations. Specifically, only hyper parameter exhibited different correlations. However, in previous work on software fairness, not all metrics have been taken into account.  This finding suggests that we need to consider different contexts in assessing the correlation between adequacy and fairness in model testing, where label bias has the most important impact.
    
\end{itemize}

To conclude, we can answer \textbf{RQ2} as:


\begin{quotebox}
   \noindent
   \textit{\textbf{RQ2:} In most cases, the adequacy metric and the fairness metric are negatively correlated. In general. The correlation between adequacy metric and fairness metric is most significant when only label bias is considered.}
\end{quotebox}
%100 sampled points using LHS without using testing methods
\subsection{RQ3: Landscape metric}
\subsubsection{method}
To answer question 3, we used Latin hypercube sampling\cite{florian1992efficient} to take 100 times for each context task and then trained the model in batches based on 12 different datasets. Thus we have a total of $3\times100\times12=3600$ applications. We conducted 10 tests for each application. For each application, we calculated the average of five adequacy metrics. Then, we investigated the ease of finding the optimal solution under different context task conditions by calculating FDC and AC.

% \begin{figure*}[t]
%      \centering
%      \begin{subfigure}[t]{0.8\textwidth}
%           \centering
%           \includegraphics[height=0.6\linewidth]{Figures/rq3_pdf/FDC.pdf}
%           \subcaption{FDC}
%      \end{subfigure}
%      \begin{subfigure}[t]{0.8\textwidth}
%           \centering
%           \includegraphics[height=0.6\linewidth]{Figures/rq3_pdf/AC.pdf}
%         \subcaption{Auto-correlation}
%      \end{subfigure}
%      \caption{RQ3, landscape analysis. (three boxes as a group: hyperparameter, label, and selection; x-axis denotes different dataset)}
%     \label{fig:corr2}
% \end{figure*}


\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{\columnwidth}
          \centering
          \includestandalone[width=\columnwidth]{Figures/rq4-1}
          %\subcaption{FDC}
     \end{subfigure}
     \vspace{-0.2cm}
     \begin{subfigure}[t]{\columnwidth}
          \centering
          \includestandalone[width=\columnwidth]{Figures/rq4-2}
        %\subcaption{Correlation Length}
     \end{subfigure}
     \caption{RQ3, landscape analysis. (three boxes as a group: hyperparameter, label, and selection; x-axis denotes different dataset)}
    \label{fig:corr2}
\end{figure}

\subsubsection{Results}

With figure~\ref{fig:corr2}, we can observe some patterns:
\begin{itemize}
    \item \textbf{Finding 4:} In most cases for FDC, label bias is closer to -1 compared to other contexts. For RQ3, the closer fdc is to -1, the closer it is to the optimal solution. In addition, for AC value, we find that its AC value is closer to 0 compared to other contexts when only hyperparameters are changed, indicating that its ruggedness is smoother. It is noteworthy that even if the landscape of instances with more tasks becomes smoother, there is no indication that these instances become easier.
    
\end{itemize}

To conclude, we can answer \textbf{RQ3} as:


\begin{quotebox}
   \noindent
   \textit{\textbf{RQ3:} In most cases, label bias is easier to find the optimal solution compared to other contexts, but it has the roughest path to find the solution. Conversely, hyperparameter has the smoothest path to find the solution, but it is more difficult to find the optimal solution.}
\end{quotebox}
